A Heterogeneous In-Memory Computing Cluster For Flexible End-to-End Inference of Real-World Deep Neural Networks

Deployment of modern TinyML tasks on small battery-constrained IoT devices requires high computational energy efficiency. Analog In-Memory Computing (IMC) using non-volatile memory (NVM) promises major efficiency improvements in deep neural network (DNN) inference and serves as on-chip memory storage for DNN weights. However, IMC's functional flexibility limitations and their impact on performance, energy, and area efficiency are not yet fully understood at the system level. To target practical end-to-end IoT applications, IMC arrays must be enclosed in heterogeneous programmable systems, introducing new system-level challenges which we aim at addressing in this work. We present a heterogeneous tightly-coupled clustered architecture integrating 8 RISC-V cores, an in-memory computing accelerator (IMA), and digital accelerators. We benchmark the system on a highly heterogeneous workload such as the Bottleneck layer from a MobileNetV2, showing 11.5x performance and 9.5x energy efficiency improvements, compared to highly optimized parallel execution on the cores. Furthermore, we explore the requirements for end-to-end inference of a full mobile-grade DNN (MobileNetV2) in terms of IMC array resources, by scaling up our heterogeneous architecture to a multi-array accelerator. Our results show that our solution, on the end-to-end inference of the MobileNetV2, is one order of magnitude better in terms of execution latency than existing programmable architectures and two orders of magnitude better than state-of-the-art heterogeneous solutions integrating in-memory computing analog cores.

==> text/01_introduction.tex <==
\section{Introduction}
% brief introduction on AIMC
Analog in-memory computing (AIMC) performs data processing in situ within memory arrays. Matrix-vector multiplication (MVM) operands can be mapped on the cross-bars of a non-volatile (NV) memory array and the \textit{dot product} operation is performed entirely in the analog domain, making IMC devices promising candidates to accelerate DNN workloads, and overcome the well-known memory bottleneck affecting traditional AI digital accelerators~\cite{InMComp}. Both charge-based memory technologies (e.g. SRAM, DRAM, and flash) and resistance-based memory technologies (e.g. RRAM, PCM, and STT-MRAM) can serve as elements for such computational units~\cite{sebastian2020memory}.
%Analog In-Memory Computing (AIMC) is an emerging paradigm holding promise to overcome the well-known von Neumann bottleneck by executing operations such as matrix-vector products in the analog domain within a crossbar arrangement, with millions of operations executed simultaneously. Both charge-based memory technologies (e.g. SRAM, DRAM, and flash), and resistance-based memory technologies (e.g. RRAM, PCM, and STT-MRAM) can serve as elements for such computational units~\cite{sebastian2020memory}.

% Demonstrations in DNN field
Several demonstrations of AIMC-based architectures have appeared in the field of Deep Neural Network (DNN) inference acceleration, showing outstanding peak energy efficiency in the order of hundreds of TOPS/W~\cite{InMComp, sebastian2020memory}. Industry interest in this technology is growing~\cite{axelera}.
An early market industrial example is represented by Mythic~\cite{mythicHC2018}, who claims efficiency of 4 TOPS/W exploiting 8b flash-based Mythic Analog Matrix Processors (MAMP) arranged as a systolic array, all connected through a mesh topology network-on-chip.
From a research perspective, several prototypes claimed tens to hundreds of TOPS/W by exploiting many different approaches, with a quite diverse set of choices in terms of numerical precision and underlying memory technologies~\cite{InMComp, sebastian2020memory}.

% What are the open challenges
However, several fundamental challenges are still open to achieve the claimed levels of efficiency at full-application scale: the intrinsic variability of analog computing both in the charge-based and resistive domain~\cite{sebastian2020memory}; difficulties in dealing with low-precision computations that are often the only ones supported by AIMC-based architectures~\cite{sebastian2020memory}; the necessity of specialized training~\cite{seb2020mixed}. Most prominently, a key issue is the limited flexibility of IMC arrays, which %is well-matched only for a limited set of primitives such as matrix-vector multiplications~\cite{InMComp}.
%As a result, most AIMC-based architectures fabricated so far have been demonstrated on trivial neural networks (up to ten layers) trained on single layers or simple data sets such as CIFAR-10 or MNIST~\cite{sebastian2020memory}, which are not representative of real-life, DNN-based applications.
%
%IMC arrays 
% the limited flexibility of AIMC-based computing
are extremely efficient on MVM or similar vector operations, but they are not flexible enough to sustain other types of workloads. To tackle this limitation, a prominent solution is to couple either general-purpose processors~\cite{jia2020programmable} or specialized digital accelerators~\cite{zhou2021analognets} with analog in-memory computing cores. This allows extending the functionality of In-Memory Accelerators (IMA), creating heterogeneous analog/digital computing fabrics, connected to the system bus~\cite{jia2020programmable}. However, this integration poses severe concerns at the system level, mainly on two aspects: bandwidth and flexibility. 

First, IMC acceleration moves the challenge towards ensuring efficient data movement within the system. In the case of volatile technologies, such as SRAM-based IMC, the weights of the DNN must be stored in non-volatile memory (external or internal to the system). This requires additional energy and time to move the data that must be stored into the cells of the IMA, anytime the cross-bar is programmed~\cite{InMComp}. When considering non-volatile technologies, such as ReRAM or PCM-based IMC arrays, weights are directly stored into the cross-bar, with no need for marshaling operations. However, previous concerns continue to affect the activations that must be moved at the boundaries of the IMC array, to perform MVMs. Taking this into account, efficient integration of IMC into heterogeneous systems requires an optimized interface design between the highly parallel IMC inputs/outputs, the programmable cores, and the rest of the system. To achieve the peak performance of the IMA without degrading its energy efficiency, the system interface must fulfill its bandwidth requirements: low bandwidth and high communication latency between the processor and the IMA might create a major bottleneck~\cite{jia2020programmable}.

Second, as a consequence of Amdahl's effect, accelerating MVM operators with an IMA moves the performance bottleneck on all the other computation needed to accomplish a certain task, which must be performed on the digital part of the system. Complex real-world neural networks mix MVMs with other workloads such as residuals, activation functions, or depth-wise convolutions; coupling the IMA with a single core, as has recently been proposed~\cite{jia2020programmable}, will likely hit Amdahl's effect, hindering by a significant factor the whole computation performance.
%Second, performing linear operators with accelerators such as IMA moves the bottleneck of the computation to the digital part. For complex tasks mixing matrix-vector multiplications with other tasks suck as residuals, activation functions, or depth-wise convolutions, augmenting the heterogeneous cluster with a single core might not be sufficient to sustain the computing requirements of IMAs~\cite{jia2020programmable}.

% Contribution
In this work, we address the system-level challenges of analog IMC by exploiting extreme heterogeneity. We propose a system architecture  based on a tightly-coupled heterogeneous cluster of fully programmable processors, analog IMC, and specialized digital accelerators. We explore the design space of such a heterogeneous cluster with the MobileNetV2 CNN, representative of a wide range of modern DNNs that leverage depthwise convolutions to reduce the size of the model by up to one order of magnitude compared to first-generation models.
%
The main contributions of this paper are the following:
\begin{itemize}
    \item We design a heterogeneous tightly-coupled shared-memory cluster that integrates 8 fully programmable RISC-V processors, an analog in-memory computing accelerator (IMA), and a dedicated digital block to accelerate depth-wise convolutions; we propose a post place\&route silicon-ready implementation targeting GlobalFoundries 22nm FDX technology;
    %\item We design a heterogeneous tightly-coupled shared-memory cluster that integrates 8 fully programmable RISC-V processors, an analog in-memory computing accelerator (IMA) and a dedicated digital block to accelerate the depth-wise convolutions;
    %\item We propose a post place\&route silicon-ready implementation of the heterogeneous analog/digital architecture targeting GlobalFoundries 22nm FDX technology;
    \item We optimize the interfaces between the analog IMA and the rest of the system to match the computing and IO requirements of the IMA, achieving performance as high as 958 GOPS on MVMs, more than 90\% of its peak theoretical throughput, overcoming by one order of magnitude other approaches where the IMA is connected through a low-bandwidth, high-latency system bus~\cite{jia2020programmable}; 
    \item We benchmark the system on a bottleneck layer, representative of modern DNNs exploiting heavily heterogeneous layers such as point-wise, depth-wise convolutions and residuals, in terms of performance and energy efficiency. The analog/digital synergistic approach demonstrates full mitigation of Amdahl's effect, showing $2.6\times$ better performance and $2.8\times$ better energy efficiency compared to executing the layers on our previous work that integrates only 8 programmable cores and the IMC analog array~\cite{ottavi2021end};
    \item We scale up the proposed system to analyze the challenges and the hardware resources necessary to enable end-to-end inference of a MobileNetV2. Our architectural paradigm executes inference in 10$ms$ with an energy of 482$\mu J$, overcoming fully digital state-of-the-art solutions~\cite{rossi2021vega} by $10\times$ in latency, reducing the energy consumption by $2.5\times$. Compared to other state-of-the-art analog/digital architectures~\cite{jia2020programmable}, our solution shows two orders of magnitude improvements in terms of execution latency.
\end{itemize}

%
These achievements demonstrate that the proposed solution is viable, paving the way to further explorations of a new generation of architectures exploiting synergies between analog and digital computing.
%
%We demonstrate that, for the heterogeneous use-case analyzed, the proposed approach improves performance by more than one order of magnitude with respect to traditional approaches where the IMA is connected through a low-bandwidth, high-latency system bus~\cite{jia2020programmable}. 
%Finally, we analyze the remaining architectural bottlenecks for MobilenetV2 execution on such a heterogeneous system. The IMA on itself can reach outstanding performance and efficiency peaks that are dictated by the size of the activated crossbar given the constant time to output for analog computations. But, the cost for auxiliary computation, data marshaling, and inefficiency of depth-wise layers from a significant constriction for efficiency (80\%) justifying the integration of specialized digital accelerators better tuned for these functions into the heterogeneous cluster.

The manuscript is organized as follows: in Sec.~\ref{sec:Related_Work} we review the state-of-the-art; in Sec.~\ref{sec:Background} we outline the background, and in Sec.~\ref{sec:BODY} we present the heterogeneous cluster architecture. Then, in Sec.~\ref{sec:Experimental_Results} and Sec.~\ref{sec:discussion} we report the experimental results, discussions, and explorations. Finally in Sec.~\ref{sec:comparison_with_soa} we compare with state-of-the-art solutions.
Sec.~\ref{sec:conclusion} concludes the paper.

==> text/02_related_work.tex <==
\section{Related Work}
\label{sec:Related_Work}
%%% technology
%Brain-inspired in-memory computing (IMC) conducts data processing in situ within the memory circuit. Matrix-vector multiplications (MVMs) operands can be mapped on the cross-bars of the memory array and the operation performed entirely in the analog domain, making IMC devices promising candidates to accelerate DNN workloads, overcoming the well-known memory bottleneck affecting traditional AI digital accelerators. 
%Analog In-Memory Computing (IMC) is an emerging paradigm holding promise to overcome the well-known von Neumann bottleneck by executing operations such as matrix-vector products in the analog domain within a crossbar arrangement, with millions of operations executed simultaneously.
Charge-based memory technologies (e.g. SRAM~\cite{biswas2018conv}, DRAM, Flash~\cite{mythicHC2018}) and non-volatile (NV) resistive memory technologies~\cite{ielmini2018memory} (e.g. ReRAM~\cite{8310400} PCM~\cite{le2020overview} and MRAM~\cite{doevenspeck2020sot}) can both serve as computing substrates for analog in-memory computing. In this section, we review the State-of-the-Art (SoA) advancements in in-memory computing technology, circuits, and systems. 
%architectures and their integration into systems dedicated to the acceleration of DNNs inference\cite{sebastian2020memory}.

%Despite floating point arithmetic is usually adopted in emerging IMC-based scientific computing applications~\cite{sebastian2019computational, le2018mixed}, for edge Artificial Intelligence (AI) applications it is usually preferable to execute the computation in the integer domain, to reduce the hardware costs and to increase the energy and area efficiency of the computation~\cite{sebastian2020memory}.
%
%To reduce the hardware costs and to increase the energy and area efficiency of the computation~\cite{sebastian2020memory}, edge Artificial Intelligence (AI) applications adopt low-bitdwidth integer arithmetic.
%
\subsubsection{IMC Arithmetic}
Low-bit-width integer computation is widely adopted in edge Artificial Intelligence (AI) applications, because of its higher efficiency and lower hardware cost than floating-point. In the IMC domain, the advantages are even more evident. Low bit-width data representation results in less area and power costs to design analog to digital (ADCs) and digital to analog (DACs) converters, which are predominant in IMC arrays~\cite{InMComp, sebastian2020memory}. The adoption of heavily quantized integer arithmetic (8-bit or less), especially for DNNs, is fully justified by the fact that Quantized Neural Networks (QNNs) show a limited drop-in Top-1 accuracy compared to the full floating-point precision model, on many AI-enhanced edge applications~\cite{jacob2018quantization}. Also, noise-robust networks are an active research field for IMC deployment~\cite{joshi2020accurate}.
%In the IMC domain, the readout circuitry to convert data from the digital/analog to analog/digital domain accounts for the major part of the power consumption of the design. Low bit-width data representation results in less area and power costs to design analog to digital converters and vice versa~\cite{InMComp, sebastian2020memory}. The adoption of heavily quantized integer arithmetic for DNN layers is fully justified by the fact that Quantized Neural Networks (QNNs) show limited drop in  Top-1 accuracy with respect to the full floating point precision model, on many AI-enhanced edge applications~\cite{jacob2018quantization, rusci2019memory}.
%Low-bit-width integer computation is more efficient than the floating point algorithms and requires less hardware. In the IMC domain, low-bit-width data representation leads The adoption of such kind of arithmetic in AI is fully justified by the fact that heavily quantized NNs have demonstrated good accuracy on many AI-enhanced edge applications, with little loss in Top-1 accuracy with respect to the same model at the full floating point precision~\cite{jacob2018quantization}.

%Charge-based memory technologies (e.g. SRAM~\cite{biswas2018conv}, DRAM, Flash~\cite{mythicHC2018} ) and resistive memory technologies~\cite{ielmini2018memory} (e.g. ReRAM~\cite{8310400} PCM~\cite{le2020overview} and MRAM~\cite{doevenspeck2020sot}) can both serve as IMC computing elements for MVMs.
%

\subsubsection{SRAM technology}
%% CIRCUITS AND ARCHITECTURES -- 
% change sentence
The SRAM technology is the most mature one, having been investigated for years to be used as volatile memory storage for digital computing architectures.
%
%Many studies have been conduced to embed computing capabilities into SRAM cells for IMC.
%
SRAMs are used to perform MVM operations both in the digital and analog domains. On one hand, in the digital domain, the computation is performed coupling SRAM cells with additional near-memory logic, such as elementary gates, full adders, or adder trees, building up a digital accelerator~\cite{chih202189tops}. On the other hand, in the analog domain, SRAMs can map MVMs by exploiting capacitive charge redistribution mechanisms along the bit-lines of the memory array~\cite{sebastian2020memory}. Compared to the analog approach, SRAM-based digital IMC provides higher robustness to noise and process, voltage, and temperature (PVT) variations, but significantly less advantages in terms of energy efficiency~\cite{ kim20191}. 
%SRAMs can perform  MVM operations both in the digital domain, coupled  with additional logic to perform the computation (such as elementary gates, full adders, adder trees)  and acting as a digital accelerator, or they can operate in the analog domain, exploiting capacitive charge redistribution mechanisms to compute MVMs along the bitlines of the memory array~\cite{sebastian2020memory}. With respect to the analog approach, SRAM-based digital IMC offers higher robustness to noise and PVT variations, but less advantages in terms of energy efficiency~\cite{chih202189tops, kim20191}. 

Most state-of-the-art academic SRAM-based IMC arrays operate in the analog domain~\cite{mittal2021survey}. One of the first prototypes appeared in 2018~\cite{biswas2018conv}, targeting binary-weight Neural Networks and demonstrating top-1 accuracy comparable with software accuracy on the MNIST dataset (~98\%). %, paving the way to further developments of SRAM-based IMC architectures.
%
SRAM-based IMC has been demonstrated for binary/ternary DNNs achieving 403 TOPS/W and software accuracy on ternary networks trained on the CIFAR-10 dataset~\cite{yin2020xnor}, as well as for reconfigurable bit-precision MVM operations showing 8 to 80 TOPS/W~\cite{yue20212, lee2020bit}. %More recent work~\cite{9094713} shows efficiency up to 672 TOPS/W and throughput of 1638 GOPS on binary-weight networks trained on CIFAR-10, exploiting 8T SRAM cells and capacitive coupling computing mechanism.
% yin et al DIGITAL- binary/ternary
%Yin et al.~\cite{yin2020xnor} for example, propose an SRAM based 256$\times$64 IMC  accelerator for binary and ternary DNNs. Prototyped in 65nm CMOS technology node, they achieve 403 TOPS/W of energy efficiency on ternary networks trained on CIFAR-10 dataset, with 88.8\% test accuracy.
% digital, bit-parallel
%Reconfigurable bit-precision multiplication and addition operations have been demonstrated on a 128kB SRAM-based IMC design in 28nm CMOS technology, showing up to 8 TOPS/W of efficiency~\cite{lee2020bit}.
%In 65nm, a recent work~\cite{yue20212} proposed a 1-to-8-bit configurable SRAM-based IMC macro, with additional ``zero-skipping`` sparsity support, showing an energy efficiency for the whole system up to 80 TOPS/W.
Other SRAM-based IMC architectures have been proposed, achieving similar accuracy and efficiency~\cite{valavi201964,  lee2021fully}.
%
The major challenge at the circuits level, which is actively being investigated in the literature, remains the computation noise that limits the signal-to-noise ration, mainly due to the sensitivity to PVT variations~\cite{sebastian2020memory}, and non-linearities~\cite{InMComp}.

\subsubsection{Resistive Memory technology}
% BEYOND SRAM -- ok rev1.0
A new generation of IMC accelerators targets emerging resistive memory technology, driven by the much higher density scaling factor that these technologies offer compared to the SRAM~\cite{roy2020memory}. 
%
Moreover, resistive memories such as Resistive RAM (ReRAM), magnetic RAM (MRAM), and phase-change memory (PCM), show other important advantages: non-volatility (NV), low power envelope, and multi-level storage~\cite{ 8310400}. IMC based on NV memories suffers from similar precision issues as SRAM-based IMCs, compounded by additional challenges coming from memristive devices, such as write variability and conductance variations (temporal and temperature-induced)~\cite{sebastian2019computational}.
%

From a system-level perspective, resistive memories serve not only as IMC primitives, but also as non-volatile storage blocks for DNN weights. This avoids moving weights across the system memory hierarchy, which is instead necessary for SRAM-based IMC. Contrarily to SRAM, re-programming the memristive cross-bars with new data during the network model execution is not affordable, due to the high latency and power consumption associated with re-writes of non-volatile memory cells, as well as their limited endurance (for ReRAM and PCM).
This forces rethinking architectures as memory-centric, with additional digital logic around to perform ancillary operations, as is the focus of this work.
%

%Although the SRAM-based IMC cross-bars seem the ones less affected from the challenges of analog non-idealities and the costs in terms of energy of the readout circuitry~\cite{InMComp}, IMC accelerators based on emerging memory technologies are coming up, driven by the much higher density scaling factor that these memory technologies offer compared to the SRAM~\cite{guo2017fast}, with additional advantages for these memories to be non-volatile, to be operated within a very low-power envelope and to enable the possibility of multilevel storage~\cite{ 8310400, xue201924}.
%. Increasing the scale of IMC based on resistive memory technologies such as resistive RAM (RRAM), magnetoresistive RAM (MRAM) and Phase Change Memory (PCM) has been demonstrated

% RERAM -- ok rev1.0
Considering ReRAM-based IMC, Chen \textit{et al.}~\cite{8310400} demonstrate significant computing parallelism, performing 8k MAC operations simultaneously. Other works show ReRAM-based IMC arrays as dense as 2Mb~\cite{9063078} or 4Mb~\cite{9365769}, with peak energy efficiencies in the range of 120-200 TOPS/W within a power envelope of few milliwatts, suitable for tiny edge AI devices. Moreover, the IMC array in~\cite{9063078}, integrated within a PCB hosting also an FPGA, runs a ResNet-20 trained on the CIFAR-10 dataset with 90\% top-1 accuracy. %Work in~\cite{liu202033} achieves similar accuracy (94\%) but on a small CNN trained on the MNIST dataset.
%On the ReRAM side, Authors in~\cite{8310400} explore various circuit-level techniques for the design of an in memory computing ReRAM-based macro, capable of performing 8k MAC operations simultaneously. The prototype in 65nm demonstrates high improvements in for ReRAM technology to be used as DNN IMC accelerator. A valuable and recent example is~\cite{liu202033}; although implemented in 130nm, the ReRAM-based IMC achieves 78.4 TOPS/W of energy efficiency on a small CNN trained on MNIST dataset with 94.4\% of accuracy. Another prototype in 22nm shows a bit re-configurable ReRAM based 4Mb IMC core, achieving a peak efficiency of 200 TOPS/W. In addition, authors in~\cite{9063078} propose a multi-bit-precision 2Mb ReRAM IMC Macro targeting tiny edge AI devices. Whithin a power envelope of few milliWatts the prototype in 22nm achieves energy efficiency of up to 120 TOPS/W and showing a 90\% top-1 accuracy of a ResNet-20 trained on the CIFAR-10 dataset. 

% MRAM -- add one paper maybe?!
For the MRAM technology, Doevenspeck \textit{et al.}~\cite{doevenspeck2020sot} present a SOT-MRAM-based IMC macro and demonstrate for the first time that resistive MRAM devices can be used for DNN applications. They claim software-like accuracy on a network targeted to the MNIST dataset.

% PCM REVIEW -- add other papers ?!
PCM-based IMC arrays have been applied in mixed-precision in-memory iterative computing, combining a computational memory unit to perform the bulk of a computational task, with a von Neumann machine, which implements a backward method to iteratively improve the accuracy of the solution. This approach has been demonstrated to solve linear equations~\cite{le2018mixed} and in DNN inference and even training tasks~\cite{sebastian2019computational}, showing limited error in the computation and much higher efficiency compared to traditional approaches~\cite{sebastian2020memory}.

Khaddam-Aljameh \textit{et al.}~\cite{hermesCor} recently presented a state-of-the-art 256$\times$256 PCM-based IMC core targeting DNN inference, fabricated in 14nm, showing energy efficiency of 10.5 TOPS/W and performance density of 1.59 TOPS/mm$^2$ on inference tasks of multi-layer perceptrons and ResNet-9 models trained on MNIST and CIFAR-10 datasets, with comparable accuracies as software baseline. In this work, we adopt the PCM-based IMC presented in~\cite{hermesCor} to carry out our experiments.

%Authors in~\cite{le2018mixed} apply successfully a PCM-based IMC array to real case-scenarios such as linear equation solving and calculation of covariance matrices using a mixed-precision approach and demonstrate negligible overall error on those use-cases with respect to software full precision computation. Targeting explicitly DNN-based tasks, it has been demonstrated that PCM-based systems can achieve significantly higher performance compared to conventional approaches for inference of DNNs and promising results for training~\cite{sebastian2019computational, giannopoulos20188}. To enforce this statement, Khaddam-Aljameh et al.~\cite{hermesCor} recently proposed a silicon prototype of a 256$\times$256 PCM-based IMC array in the 14nm technology node. They are able to demonstrate the highest throughput of 1 TOPS on CIFAR-10 inference tasks with respect to other solutions based on SRAM and MRAM, with energy efficiency of 10.5 TOPS/W and a performance density of 1.59 TOPS/mm$^2$. Also, they claim training accuracy close to full-precision software accuracy for MLP and ResNet-9 networks trained on MNIST and CIFAR-10 datasets. 

%\subsection{Training}
%% TRAINING ALGORITHMS ADVANCEMENTS
%Training large DNN models to be deployed on IMC arrays is challenging, due to their noise and output variability, which significantly affect the accuracy outcome of the models. Having as main focus performance and efficiency rather than the training itself, circuits presented above are demonstrated only for small networks, trained on trivial datasets, not representative of modern AI-enhanced edge applications.

%Nevertheless, recent efforts are progressing in literature to accurately model the analog noise components to be included in the training procedure~\cite{garcia2020training, ambrogio2018equivalent, rekhi2019analog} as well as specific training strategies and custom DNN architectures to address both analog-based training and extremely quantized data representation~\cite{zhou2021analognets}.

%While motivated by unprecedent throughput and efficiency, one of the open challenges of emerging IMC arrays for DNN tasks is that analog non-idealities such as devices variability, drifting and non-idealities of the read-out circuitry, strongly influences the accuracy outcome of the training flows, limiting the deployment of real-sized neural networks on such architectures. Focused mostly on performance and efficiency numbers, all the contributions presented above are demonstrated only on small networks that are not representative of modern DNN-enhanced applications. 


\subsubsection{Architectures and Systems}
%% LIMITS OF IMC ACCELERATORS AND HETEROGENEOUS SYSTEMS
As discussed, there are several challenges related to technology that affect both charge-based and resistive IMC circuits currently under scrutiny from researchers. However, provided that these issues can be solved, another essential challenge is the integration of in-memory computational primitives into heterogeneous systems.
In this work, we focus in particular on this aspect.

IMC cores primarily target matrix-vector multiplications (MVMs) or other similar vector operations, showing incredible throughput and efficiency. Although MVM operations are predominant in modern DNNs, they still represent only a subset of the DNN computation~\cite{8502276}, which also includes residual connections, pooling layers, non-linear activation functions, softmax, etc.. Increasing the throughput of MVMs with IMC moves the performance bottleneck to all the other layers, which can not be easily mapped on IMC arrays. From a broader application perspective, an edge-computing system might incur workloads characteristically different than MVMs, such as data management and control tasks that are performed together with neural tasks~\cite{pulp_frontnet}. It is necessary, for a complete architecture, to address this computation in a programmable way. This reasoning strongly motivates the integration of the IMC with other specialized accelerators and software programmable cores in heterogeneous architectures~\cite{InMComp}.


%As discussed above, there are open challenges at the technological, circuit and training level that are actively investigated in the literature. However, in this work we tackle mainly the challenges that the in-memory computing paradigm shows at the system-level. IMC cores primarily target matrix-vector multiplications (MVMs) or other similar vector operations. They show incredible throughput and efficiency on this type of kernels, but they are not flexible to support different types of workloads. Although MVM operations are predominant in modern DNNs, they represent only a subset of the computation~\cite{8502276}, with other subsets to be residual connections, pooling layers, non-linear activation functions. Increasing the throughput of MVMs with IMC moves the performance bottleneck on these layers. Furthermore, from a broader practical application perspective, DNN tasks are not the only type of workload that a computing platform might incur in: data management, control tasks, peripheral managements are some examples. For these reasons, edge computing systems should target a wider-range of workloads that might be characteristically different than MVMs, where the emphasis on data movement that motivates IMC might be reduced. 
%

%removed this dazzi2021accelerating
To the best of our knowledge, not many works specifically focused on the integration of IMC arrays in heterogeneous analog/digital systems have been presented in literature so far. Dazzi~\textit{et al.}~\cite{ dazzi2021efficient} propose more advanced IMC multi-core approaches with very carefully staged core-to-core dataflow, but the focus is mostly on convolutions and there are no provisions for heterogeneous computing nor for computations that do not map efficiently on the AIMC arrays.

% 1st example
%An early market example of a heterogeneous system is Mythic~\cite{mythicHC2018}, which complements an 8-bit compute capable analog flash array with a RISC-V microcontroller and a dedicated SIMD engine, integrated with a Network-on-Chip and an SRAM storage block. The company claims that the prototype runs within an envelope of 5W, capable of executing the ResNet-50 network using 5MB of on-chip SRAM, achieving energy efficiency of up to 4 TOPS/W.
% 2nd example: arm+ibm
Zhou~\textit{et al.}~\cite{zhou2021analognets} propose a PCM-based IMC array modeled in 14nm technology, complemented with additional digital logic that that performs activation and pooling operations. A small SRAM memory acts then as a layer-to-layer intermediate buffer, followed by a hardware block that handles \textsc{im2col} transformations. The proposed solution is capable of performing 8/6/4-bit$\times$8-bit matrix-vector multiplications achieving a peak efficiency of 112 TOPS/W. The authors demonstrate the system on a small end-to-end inference of a custom DNN model, with  95.6\% of accuracy, at a performance of 7.7 inf/s with 8.22 $\mu J / inf$. However, this type of architecture is not flexible enough to support heterogeneous workloads, since it does not feature programmable cores.
% 3rd example: jia et al.

Jia~\textit{et al.}~\cite{new_verma} propose a 4$\times$4 array of cores consisting of charge-based IMC cross-bars extended with a programmable near-memory-computing (NMC) digital accelerator that performs single-instruction-multiple-data (SIMD) computing, shifting, pooling, and activation functions. On 8-bit MVMs, the prototype in 16nm shows 3 TOPS of peak performance with 30 TOPS/W of efficiency. Coupled with off-chip FPGA and MCU that handle communication with a host PC and control flows, the prototype has been demonstrated on a ResNet-50 model with 4-bit weights and activations, achieving a peak performance of 3.4 TOPS.

An example of a heterogeneous system is given by~\cite{jia2020programmable}, which presents a silicon prototype in 65-nm CMOS that integrates a charge-domain compute-in-memory unit supporting 1to8-bit$\times$1to8-bit matrix-vector multiplications, into a tiny RISC-V CPU enriched with a direct memory access controller (DMA) and a set of peripherals. The results show a peak efficiency of 400 TOPS/W at 1b configuration on the end-to-end inference of a small CIFAR-10 ten-layers network. However, also in this case the architecture can not afford complex heterogeneous computation: the core delivers only a few million operations per second and it can only be used for control tasks such as programming DMA transfers, not being capable of performing compute-intensive functions with a reasonable performance level.
%
%Another example is~\cite{zhou2021analognets}, in which the authors present an application-specific system that features an IMC array plus a digital activation processing and storage pipeline. The system is capable of performing 8-6-4b$\times$4b matrix-vector multiplications achieving a peak efficiency of 112 TOPS/W. Demonstrated on a custom built network, namely AnalogNet, the system is able of executing the keyword-spotting task with 95.6\% of accuracy, at a performance of 7.7 inf/s with 8.22 $\mu J / inf$.   

The limits of the above-mentioned systems are mainly two: first, the integration of the IMC accelerator (IMA) is loosely-coupled, with the IMA connected with other cores through a low bandwidth, high latency system bus; second, the presented heterogeneous systems are demonstrated either on trivial neural networks model of few layers (trained on simple datasets such as CIFAR-10 or MNIST) or on custom NN model built ad-hoc to fit the requirements of the architecture. Neither approach is representative of modern DNN models widely used in classification and detection tasks at the edge of the IoT. 
% this wor

In this manuscript, we extend the work we presented in~\cite{ottavi2021end} by coupling the IMA with a novel design of a digital accelerator to improve the efficiency of depth-wise kernels, integrated into the heterogeneous system and we fully implement the cluster in the GlobalFoundries 22nm FDX technology. Furthermore, we scale up the architecture and explore the resources necessary to enable the end-to-end inference of a full MobileNetV2 network, a much more realistic benchmark for the class of networks that an ultra-low-power IoT end-node could target.

%we include a new model of the PCM-based IMC array, characterized from the measurements of a silicon prototype~\cite{hermesCor};

%In this work we deeply analyze the challenges of integrating analog IMC accelerator into digital systems, to enable end-to-end inference of modern neural network topologies (such as the MobileNetV2). As the result of our explorations we propose the integration of an IMC accelerator based on the PCM technology into a tightly-coupled parallel cluster of 8 RISC-V processors and additional dedicated digital accelerators, extending the analysis conduced in~\cite{ottavi2021end}.
%%% TO COMPLETE
%We propose an exhaustive architectural design space explorations targeting the Bottleneck layer of the MobileNetV2 as reference benchmark, representative of a wide range of modern DNNs leveraging depth-wise convolutions~\cite{li2020micronet, DBLP}, achieving a peak performance of 958 TOPS with an efficiency of 6.3 TOPS/W.
%
%To put out results in perspective we end the manuscript with a discussion on the system scalability. We investigate the hardware resources required at the architectural level to enable end-to-end inference of a MobilenetV2, and we show that the integration of in-memory analog cores into digital tightly-coupled multi-core cluster pushes at least by 10$\times$ the inference speed, compared to state-of-the-art digital solutions.

==> text/03_background.tex <==
\section{Background}
\label{sec:Background}

\subsection{PCM-based In-Memory Accelerator}
\label{sec:in-mem_comp}
% In this section, we describe the basic operations of the PCM in-memory crossbar array used in this work.
In this paper, we use the In-Memory Computing accelerator presented in~\cite{hermesCor} which is based on a Phase-Change Memory (PCM) cross-bar. In this architecture, the memory devices are resistors with programmable conductance placed at the crosspoints of a 2D array with one terminal connected to horizontal wires called \textit{word-lines} and the other terminal connected to vertical wires called \textit{bit-lines}, enabling the execution of several computational primitives concurrently.

%To perform the MVM operation between the matrix $\mathbf{A}$ and the vector $\mathbf{x}$, the elements $\mathbf{A}_{ij}$ of $\mathbf{A}$ are linearly mapped to the conductance values of two PCM devices in a differential way, with a precision of 4 bits (signed). (to denote a signed weight...)

%The In-Memory Computing accelerator used in this paper is based on a Phase-Change Memory (PCM) crossbar array~\cite{hermesCor}. In this architecture, the memory devices are resistors with programmable conductance placed at the crosspoints of a 2D array with one terminal connected to horizontal wires called \textit{word-lines} and the other terminal connected to vertical wires called \textit{bit-lines}, enabling the execution of several computational primitives concurrently.

To perform the product of a matrix $\mathbf{A}$ by a vector $\mathbf{x}$, the PCM devices are programmed with conductance values proportional to the values $\mathbf{A}_{ij}$ of $\mathbf{A}$, with a precision of 4-bit (signed). Then the word-lines are driven with voltage pulses, whose duration are proportional to $\mathbf{x}_j$, using a set of digital-to-analog converters (DACs) with 8 bits of precision (signed). By Ohm's law, each PCM device contributes a current proportional to $\mathbf{A}_{ij}\cdot\mathbf{x}_j$ on the $i$-th bit-line, resulting in a total integrated current proportional to the dot product $\mathbf{y}_i = \sum_j \mathbf{A}_{ij}\cdot\mathbf{x}_j$. At the end of each bit-line, there is an analog-to-digital converter (ADC) used to sample the bit-line current and convert it into an 8-bit digital value (signed).

For DNN inference, the $\mathbf{A}$ matrix can be used to store the weights of the linear part of a Fully Connected, Convolutional, or Depthwise Convolutional layer. Note that typically 2 PCM devices are used to denote a signed weight~\cite{Y2020joshiNatComm}. In conventional digital architectures, the dot product of 4-bit weights and 8-bit input activations requires a high-precision intermediate representation (often, 32 bits) that is subject to scaling, clipping, and quantization to produce a vector of 8-bit output activations~\cite{burrello2020dory}. In the IMC cross-bar, instead, the intermediate representation is an analog current, while scaling, clipping, and quantization are performed directly by the bit-line ADCs by setting appropriate current limits. Recent work has shown that it is possible to achieve software-equivalent classification accuracy using this approach~\cite{Y2020joshiNatComm}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{images/acc_integration_cluster.pdf}
    \caption{Overview of the PULP cluster architecture, integrating the IMA and the digital depth-wise accelerator. Each accelerator is enclosed into a Hardware Processing Engine (HWPE) subsystem, depicted on the right.}
    \label{fig:cluster_archi}
\end{figure*}
\subsection{The PULP Cluster}

Highly parallelizable workloads such as DNNs are a perfect fit for high core count heterogeneous systems that can integrate specialized accelerators. We base our work on the PULP cluster~\cite{rossi2021vega}, an open-source computing platform leveraging parallelism and architectural heterogeneity.
%
The PULP cluster we assume as a reference is depicted on the left side of  Fig.~\ref{fig:cluster_archi}. It incorporates 8 RISC-V cores, each featuring a 4-stage in-order single-issue pipeline and implementing the RISC-V RV32IMCXpulpV2 Instruction Set Architecture (ISA).  XpulpV2 is a custom extension to the RISC-V ISA~\cite{gautschi2017near} meant to accelerate arithmetic intensive kernels.
%

The cores of the baseline cluster communicate through a shared and word interleaved memory called Tightly Coupled Data Memory (TCDM), referred to as L1 memory. The size of the memory is parametrizable and, in the implementation of the cluster used in this work, is 512 kB, divided on multiple banks with a banking factor of four with respect to the number of cores (i.e., 32 banks for the 8-cores configuration). The cores access the memory through a low latency logarithmic interconnect (LIC), that serves the memory accesses in one cycle. 
%
The cluster workload can be offloaded to accelerators, integrated into the cluster through a standardized interface~\cite{conti2015ultra}, discussed in Section \ref{sec:HWPE}. %  that is customizable to accommodate the specifications of the accelerator itself. HWPEs, depicted in the right side of Fig.~\ref{fig:cluster_archi}, expose a control interface to the cluster cores through which the accelerators can be programmed and an inititiator wide-bitwidth data interface towards the TCDM to bring data in and out the data-path of the accelerator. 
% 

The cluster communicates with a micro-controller system that handles input/output peripherals, through an AXI interface. Moreover, it is served with a DMA controller dedicated to the data transfers between the TCDM and the second level of memory, hosted by the micro-controller system, which also contains the program instructions for the cluster cores. 
%
Each core fetches the instructions from a hierarchical instruction cache organized on two levels (the first private to each core, the second shared) to optimize the hit rate. 
%
The cluster is also supported by a Hardware Synchronization Unit that manages synchronization and thread dispatching, enabling low-overhead and fine-grained parallelism, thus high energy efficiency: each core or accelerator waiting for a barrier, or more in general for a custom event, is brought into a fully clock gated state.


%\subsection{Hardware Processing Engine (HWPE)}
%\label{sec:HWPE_background}

%\subsection{Heterogeneous Cluster Interconnect}
%\label{sec:HCI_background}
%The Heterogeneous Cluster Interconnect (HCI) is a single-cycle latency interconnect designed for synergistic operations of the RISC-V cores with hardware accelerators integrated via the HWPE interface. 
%
%The HCI is divided into two branches, \textit{logarithmic} and \textit{shallow}: the logarithmic branch allows all-to-all single-cycle access from a 32-bit initiator port (from the cores or DMA) to each of the word-interleaved memory banks; eventual conflicts for accesses on the same memory bank are managed granting access to only one initiator, with a round-robin arbitration scheme. 
%
%The \textit{shallow} branch consists of a  $Width_{shallow}$ width-parametric single port (i.e. 512 bits wide port, in the context of this work), routed to $N_{shallow}$ adjacent memory banks treated like a single bank of  $Width_{shallow}$ bus width, without arbitration.
%
%The TCDM banks are connected to the two branches through a set of multiplexers, which grant access to one branch or the other according to a configurable-latency starvation-free rotation scheme. 

==> text/04_body.tex <==
\section{Heterogeneous System}
In this section we present the IMA sub-system, the depth-wise digital accelerator and their integration into the PULP cluster. We end the section with a short description of the accelerators' programming paradigm.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IMA ACCELERATOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IMA Subsystem Architecture}
\label{sec:execution_model}
\label{sec:ima_description}

In this section we describe the integration of the PCM-based IMC cross-bar accelerator, introduced in the section \ref{sec:in-mem_comp}, into the PULP cluster.

% IMA sub-system
\begin{figure}[t]
\centerline{\includegraphics[width=0.5\textwidth]{images/old_paper/ima_subsystem_2.png}}
\caption{IMA Subsystem in a PULP cluster. The subsystem can be configured at design time to support a total of $2\times N$ 32-bit ports towards TCDM, evenly split between load and store units connected directly to the PCM array by means of DACs and ADCs, respectively.}
\label{fig:ima_subsystem}
\end{figure}

% IMA Timeline
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\linewidth]{images/IMA_execution_model.pdf}
\caption{IMA mapping of standard convolutions on the PCM crossbar. Below the timeline of the two execution models.}
\label{fig:ima_map_plus_timeline}
\end{figure}

%Why we integrate the xbar into hwpe
To amplify the performance and the energy efficiency of the IMC cross-bar on data movements, and to ease its integration into the PULP cluster, we incorporate the cross-bar within a standardized Hardware Processing Engine (HWPE) interface~\footnote{https://hwpe-doc.readthedocs.io/en/latest/} which exposes a control and a data interface towards the rest of the cluster. This sub-system, depicted in Fig.~\ref{fig:ima_subsystem}, is called In-Memory Accelerator (IMA). 

% explanation of data and ctrl intf
The control interface allows the clusters cores to access the IMA registers for configuration. The data interface is directly connected to the TCDM memory through the master ports of the logarithmic interconnect (LIC), the same used by the cores of the cluster. The width of the IMA data bus is a design-time parameter that can be chosen depending on the required bandwidth,  as we show in Section~\ref{sec:IMC_Accelerator_Performance},~\ref{sec:bottlenecs_res}, while the TCDM memory is 512kB in size, spread over 32 banks with 32-bits data bus width.

% main hw blocks of the IMA, the Controller, The Engine
The IMA accelerator consists of three fundamental blocks. The \textit{Controller}, which can be targeted in a memory-mapped fashion via the control port, is responsible of coordinating the overall operation of the accelerator. It contains a latch-based register file that stores the user execution configuration and a central controller \textit{finite-state-machine} (FSM) which coordinates the other blocks. The \textit{Engine} contains both the digital and analog parts of the IMA data-path. The digital part is composed of buffers for ADCs and DACs and control circuitry; the analog core encloses all the PCM devices (including PCM programming circuitry), as well as the ADCs and DACs themselves. 

% The streamer
The \textit{Streamer} contains the blocks necessary to move inputs and results in and out of the accelerator through its master port of the data interface and transform the memory accesses into coherent streams to feed the accelerator engine. The streams are organized in two separated modules, namely \textit{source} for the in-coming one (for the inputs and or weights during the programming phase of the analog cross-bar) and \textit{sink} for the out-coming one (for the results). Both source and sink include a three-dimensional address generator to start the memory transactions and a re-aligner module to form word-aligned streams from non-word-aligned memory accesses, without constraining the outside memory system to support misaligned accesses. The memory accesses generated by the two streams are dynamically multiplexed towards the data interface. Such a choice avoids the duplication of the data interface ports while not causing any performance overhead; eventual contentions are efficiently solved by a round-robin mechanism.

% Configuration of the IMA and programming of the regs
The configuration sequence of the IMA starts when a core acquires a lock over the accelerator by reading a special \textsc{acquire} register through the peripheral control interface. After that, the core can interact with the IMA by: programming the PCM devices with the weights of one or multiple layers; reading the conductance value of a PCM device; configuring a \textit{job} by setting the address of input and output data in TCDM and the ADC configuration; when the configuration is over the job can be started by writing to a special \textsc{trigger} register.
To minimize the IMA configuration and synchronization overhead, multiple jobs can be pipelined by setting the register file with the correct strides. Thanks to the \textsc{inter-job pipeline}, a whole layer can be executed with only one configuration phase.
% IMA Data layout
The IMA works on input data stored in L1 with the HWC format, i.e., with consecutive data elements encoding pixels that are adjacent in the channel dimension. In Fig.~\ref{fig:ima_map_plus_timeline}, we show how a CNN layer is mapped on the IMA array.

% Two exec. models: sequential and pipelined 
We design, analyze and compare two execution models of the single job. The first one splits the execution of the job into three phases operated sequentially. \textsc{stream-in}: fetch data from the TCDM that is then streamed to the engine's internal DACs buffers; \textsc{computation}: analog computation on the crossbar and writing of the ADCs buffers; \textsc{stream-out}: stream data from buffers back to the TCDM. As we demonstrate in section \ref{sec:IMC_Accelerator_Performance}, this model under-utilizes the band-width of the system, strongly limiting the peak performance of the IMA. As a solution, we propose a pipelined execution model of the job, where the three aforementioned phases can overlap each other at the cost of additional hardware resources: we add two pipeline registers before and after the DACs and ADCs buffers and we extend the \textit{Engine} FSM with additional states to control the overlapping phases. 

% Explanation of the pipeline
The timeline of the execution is reported in Fig.~\ref{fig:ima_map_plus_timeline}. Before staring the computation, the single-cycle \textsc{push} state move forward the pipeline, pushing the data from the input pipeline registers to the DAC buffers and from the ADC buffers to the output pipeline registers. During the computation of the $i-th$ job (if not the last one to compute), the \textit{engine} FSM enters the \textsc{COMP. ST-IN} state and sets the streamer to start streaming in the inputs for the successive $(i+1)-th$ job . When the stream-in phase has finished, if there are the results of the previous job to stream-out, the \textit{engine} FSM enters the \textsc{COMP. ST-OUT} state to configure the stream. As a design choice, the stream-in phase always has highest priority over the stream-out, without impacting the execution performance. As soon as the current computation finishes ($i-th$ job), a new \textsc{push} cycle refreshes the pipeline moving the data forward. If we consider only the digital logic of the IMA, the pipelined approach increases the area by about 40\%, due to the doubled number of input/output registers. However, this overhead reduces to 5\% if we consider the total area of the accelerator (digital logic and analog IMC cross-bar), with respect to the implementation of the sequential approach. 
 
% further details on the computing model of the IMA
For a standard convolutional layer, the \textsc{stream-in} phase also includes a virtual \textsc{IM2COL} transformation~\cite{garofalo2020pulp}, which is performed directly by the streamers, enabling to remap all computation supported by the IMA to matrix-vector products of the form discussed in Section~\ref{sec:in-mem_comp}.
As a consequence, the PCM array computes $C_{out}$ output feature maps from a complete input volume of $C_{in}\times K\times K$ pixels in a single operation, where $C_{in,out}$ indicate the number of channels and $K$ is the filter size.


% ancillary contribution to reduce power. Consider whether to remove it or not
To reduce the power consumption of the cluster on DNN layers offloaded to the IMA, the top interface is extended with an end of computation (\textit{Eoc\_event}) signal. After programming the IMA and starting its execution, the core in the cluster goes in sleep mode, with its clock and fetch\_enable signal disabled. It is woken up by the Event Unit once it has been notified by the IMA with the \textit{Eoc\_event} signal. This event is raised by the controller FSM of the IMA when all the pipelined jobs have finished the execution. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DW ACCELERATOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dedicated Depth-Wise Digital Accelerator}
\label{sec:dw_accelerator_archi}

% Depth-wise accelerator architecture
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/DW_architecture_v1.pdf}
    \caption{Architecture overview of the Dwpth-wise digital accelerator. (a) The figure shows the main overview of the accelerator, consistins of three main blocks: the \textit{Streamer} interfaces the accelerator with the cluster memory, the \textit{Controller} handles the execution and and the \textit{Engine}, which contains the datapath. (b) The figure shows with more detail how the depth-wise operation is executed on the accelerator, highlighting its peculiarity. The MAC unit executes one 3$\times$3$\times$4}
    \label{fig:dw_archi}
\end{figure}

% Why we design a custom accelerator for the depth-wise
Depth-wise (DW) convolutions have been introduced to shrink the model size of the neural networks and their computational cost, due to their higher parameter efficiency \cite{DBLP}. Due to their higher parameters sparsity level (each output channel depends only on the corresponding input channel) compared to the standard 3-D convolution, DW layers are very inefficient to be mapped on IMC arrays, as we show in section \ref{sec:IMC_Accelerator_Performance}, causing huge performance degradation of the overall system when running Bottleneck layers. To speed-up the execution of the depth-wise layers, we design a custom digital accelerator and we integrate it into the heterogeneous cluster, already integrating the IMA.

% Brief description of the features of the accelerator
The DW accelerator we propose in this work is capable of processing input tensors and weights at the precision of 8-bits, accumulating the results in intermediate 32-bit registers and performing non-linear activation functions such as ReLu and a set of ancillary functions (i.e. shifting and clipping) to bring back the final result into the 8-bit precision.
%
Figure \ref{fig:dw_archi} shows the general architecture of the proposed accelerator. It consists of three main blocks: the \textit{Controller}, the \textit{streamer}, the \textit{Engine}. 

% THE STREAMER
The \textit{Streamer} acts as address generator to access the TCDM memory and reorganize the memory accesses in input streams to be sent to the \textit{Engine}, eventually re-aligning misaligned accesses to the memory. The same but in the opposite way happens for the output streams. To reduce area and power consumption, the accesses from and to the TCDM memory are dinamically muxed into a single 128-bit wide bus, which is exposed to the rest of the system via the HWPE data interface, on the same trail of the streamer presented in section \ref{sec:ima_description}. Intermediate FIFOs in both directions are used to decouple the streams from eventual memory contentions.

%THE CONTROLLER
The \textit{Controller} is exposed to the rest of the system through memory-mapped latch-based registers that are used to configure the DW execution. It contains two sets of registers: the \textit{job-dependent} ones are used to configure the pointers to access the input tensors and the weights, residing in the TCDM memory, and the memory address to store the output feature map and they normally change betweend multiple-jobs execution. Also, registers to configure three-dimensional strides and number of memory accesses are used to program the address generator of the \textit{streamer} and allow to access non-contiguous memory elements. Additional \textit{generic} registers host parameters that are assumed to be static between the execution of multiple jobs such as to enable or disable ReLu, clipping and to program the amount of shifting on the intermediate MAC results and normally they are static. In the current design, the main limitation is that it is not possible to configure the stride and the size of the window filter, which are hardwired inside the engine to stride 1 and 3$\times$3 filters, respectively. The FSM of this block orchestrates the interaction among the three main blocks and supervise the execution phases of the accelerator.

% THE ENGINE
The \textit{Engine} contains the datapath of the accelerator, consisting of two intermediate buffers to store weights and activations to be used during the current operation, a network of Multiply-and-Accumulate (MAC) and ancillary blocks to compute ReLu, shifting and clipping operations, as shown in Figure. The DW kernel computation is controlled by a small FSM.
 
% Data-flow 
The computing data-flow of the depth-wise accelerator is weight-stationary. The weights from 16 different filters, assumed to be 8-bit signed elements, are loaded from the TCDM memory at the beginning of the computation, sign-extended and stored into the weight buffer that features 3x3x16 registers of 9-bits. 
% Weight buffer
The weights reside into the buffer for the whole duration of a job, the cycles necessary to scan the input feature map in its all spatial dimension and the corresponding channels to the sets of weights used. At the end of the job, the FSM notifies the \textit{Controller} and the \textit{Streamer} that a new stream is necessary to update the DW filters. 
% Window buffer
The input tensor scan procedure consists of a sliding window mechanism implemented in the window buffer. To this purpose, the buffer hosts 3x3x16 8-bits registers that contain the current image used in the convolution plus an additional row of 3x16 bytes.
% Computing paradigm and the pipelined approach
To reduce the latency of the execution, the DW Accelerator supports pipelined jobs but also pipelined intra-job computing phases. During the MAC evaluation phase, the window buffer is allowed to request new streams to fill the additional row in the buffer, overlapping the streams to the computing phase. At the next MAC evaluation, the window to be convolved with the filters is obtained shifting by one row down the previous window and reusing two lines of it, increasing the data reuse rate. Such a mechanism is performed until the scan operation reaches one spatial edge of the image. In this case, a \textit{clear} operation on the entire window buffer is needed. Despite the penalty of fetching the whole window from the memory whenever an edge of the input image is reached, we measure that our approach reduces the memory accesses by more than 60\% (e.g. simple estimates on a 28$\times$28 image would result in 65\% of memory access savings with the discussed approach). (Serve una figura)

% conclusive sentence of the pipeline (dynamic mux)
To reduce the execution cycles, also the output streams can overlap the execution phase or the stream-in phase. In this case, the dynamic multiplexer (that muxes the two streams) handles the eventual concurrent access to the master port of the data interface towards the TCDM through a round-robin arbitration mechanism. From an empiric evaluation on the layers benchmarked in this work, no stalls or loss of performance are observed with the presented dynamic approach.

% MAC Units
The MAC unit represents the core of the computation. It consits of 36 multipliers and a reduction tree that can compute an output block of 3$\times$3$\times$4 intermediate output pixels in one cycle. Given the size of the window and weight buffer, the MAC un.
From the window buffer a chunk of 3x3x4 elements is loaded and multiplied pixel-by-pixel with the weights of the weight buffer. Per each pixel of a given channel. The intermediate multiply results are reduced through a sum-tree to produce one pixel per row, corresponding to the output pixel of a given channel and stored in a 32-bit multi-dimensional array. The reduced results are then passed through the ReLu block. If activated by the configuration phase, the ReLu cuts off all the negative results. The last stage of the computation consists of a shifting and clipping operation to bring back the results into an 8-bit range. Once this is completed all the 16 channels are stored into the memory through a stream request.  

\subsection{Integration of the Accelerators and Programming Model}

% Small recap of how the two accelerators are connected into the cluster
The heterogeneous cluster is reported in Fig.\ref{fig:cluster_archi}. To reduce the area overhead and the logarithmic interconnect arbitration latency, the data interface of the IMA and the DW-subsystem are statically multiplexed towards the TCDM. This choice does not cause any performance degradation, since in our computing model the depth-wise accelerator and the IMA can not be active concurrently. However, they can be programmed individually by the clusters cores. Each accelerator has its own programming bus and the configuration registers are mapped in different regions of the cluster memory map. To ease the programming phase of the accelerators we expose to the programmer a set of hardware-abstraction-layer (hal) functions that can be inferred directly into the C code through their explicit invocations.

==> text/04_body_v2.tex <==
\section{Heterogeneous System}
\label{sec:BODY}
In this section, we present the analog in-memory accelerator (IMA), the depth-wise digital accelerator, and their integration into the PULP cluster through a standardized interface called Hardware Processing Engine.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% INTEGRATION AND HWPE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hardware Processing Engines}
\label{sec:HWPE}
% General info on HWPE
To improve the performance and the energy efficiency of the accelerators in data movement operations, and to ease their integration into the cluster, each of the two accelerators presented in this work is incorporated as a Hardware Processing Engine (HWPE) using a standardized interface\footnote{https://hwpe-doc.readthedocs.io/en/latest/}. HWPEs expose a control and a data interface towards the rest of the cluster. The control interface allows the cluster's cores to access the registers of the targeted accelerator for configuration. The data interface is connected to the TCDM memory through multiple master ports on the logarithmic interconnect, similarly to what happens with the cores of the cluster. The width of this bus is a design-time parameter and can be chosen depending on the required bandwidth of the accelerator. 

% Integration and muxing
Fig.\ref{fig:cluster_archi} shows the heterogeneous cluster with two distinct HWPE interfaces encapsulating the IMA (namely \textit{IMA subsystem}) and the depth-wise accelerator (namely \textit{DW subsystem}). To avoid a large increase in the area of the logarithmic interconnect and in the latency of its arbitration scheme, the data interface of the \textit{IMA subsystem} and the \textit{DW subsystem} are statically multiplexed towards the TCDM, sharing the same physical ports on the interconnect. The two accelerators are used in a time-interleaved fashion, allowing one accelerator full access to the TCDM at a time. This choice does not cause any performance degradation, since in our DNN computing model the depth-wise accelerator and the IMA can not be active concurrently. However, they can be programmed individually by the cores of the clusters. Each accelerator has its own programming bus and the configuration registers are mapped in different regions of the cluster memory map. To ease the programming phase of the accelerators, we expose to the programmer a set of hardware-abstraction-layer (HAL) functions that can be inferred directly into the C code through their explicit invocations.
To reduce the power consumption of the cluster on jobs deployed to HWPEs, the latter expose an end of computation signal towards the cluster.
After programming the HWPE and triggering its execution, the cluster cores can enter a low-power clock-gated sleep mode. Once the HWPE notifies an end of computation signal, the core can be woken up by the cluster Event Unit  

% From the inside...
From the inside, HWPEs consist of three main blocks: the \textit{Controller}, the \textit{Engine}, and the \textit{Streamer}.
% The controller
The \textit{Controller} contains a memory-mapped latch-based register file, that is used to configure the execution of the accelerator, and the main \textit{Finite-State-Machine} (FSM) of the HWPE system, that coordinates the other blocks. The \textit{Controller} can be targeted by the cores of the cluster in a memory-mapped fashion via the control interface introduced above. The semantic and the number of registers as well as the FSM are customized to accommodate the requirements of the enclosed accelerator. 
% The Engine
The \textit{Engine} contains the data path of the accelerator and the specific FSM that coordinates the execution flow. It is, therefore, highly dependent on the specific accelerator design.

% The streamer
The \textit{Streamer} contains the blocks necessary to move inputs and results in and out of the accelerator through its master port of the data interface and transform the memory accesses into coherent streams to feed the accelerator \textit{Engine}. The streams are organized in two separated modules, namely \textit{source} for incoming streams and \textit{sink} for the outgoing ones. Both \textit{source} and \textit{sink} include address generators capable to generate three-dimensional access patterns in TCDM with configurable strides. They also include a re-aligner module to form word-aligned streams from non-word-aligned memory accesses, without constraining the memory system outside the HWPE to support misaligned accesses. The memory accesses generated by the two streams are dynamically multiplexed towards the data interface. Such a choice avoids the duplication of the data interface ports while not causing any performance overhead; eventual contentions are efficiently solved by an arbiter featuring a round-robin arbitration policy. Intermediate FIFOs in both directions are used to decouple the streams from eventual memory contentions and release the pressure on timing closure of the tightly-coupled system.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IMA ACCELERATOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IMA Subsystem Architecture}
\label{sec:execution_model}
\label{sec:ima_description}

% IMA sub-system
\begin{figure}[t]
\centerline{\includegraphics[width=0.75\linewidth]{images/IMA_subsystem.pdf}}
\caption{IMA enclosed into the HWPE interface. The \textit{data\_itf} width is designed to match the IO requirements of the IMA.}
\label{fig:ima_subsystem}
\end{figure}

% IMA Timeline
\begin{figure}[!t]
\centering
\includegraphics[width=0.95\linewidth]{images/IMA_execution_model.pdf}
\caption{(a) Mapping of standard convolutions on the PCM crossbar. (b) Timeline of the sequential and pipelined execution models.}
\label{fig:ima_map_plus_timeline}
\end{figure}

%Why we integrate the xbar into hwpe
Fig.~\ref{fig:ima_subsystem} shows the integration of the IMC cross-bar within the HWPE.
% explanation of data and ctrl intf
The width of the IMA data interface is sized to sustain the bandwidth requirements of the analog core, as shown in Section~\ref{sec:IMC_Accelerator_Performance}.
% main hw blocks of the IMA, the Controller, The Engine
The \textit{Engine} contains both the digital and analog parts of the IMA data path. The digital part is composed of buffers for ADCs and DACs and of control circuitry; the analog core encloses all the PCM devices (including PCM programming circuitry), as well as the ADCs and DACs themselves. 

% ima data layout, how the conv is mapped on the ima, 
% IMA Data layout
The IMA works on input data stored in L1 with the HWC format, i.e., with consecutive data elements encoding pixels that are adjacent in the channel dimension. In Fig.~\ref{fig:ima_map_plus_timeline}, we show how a CNN layer is mapped on the IMA array.
% further details on the computing model of the IMA
For a standard convolutional layer, the streamers can directly perform a virtual \textsc{im2col} transformation~\cite{garofalo2020pulp}, enabling to remap all computation supported by the IMA to matrix-vector products of the form discussed in Section~\ref{sec:in-mem_comp}. As a consequence, the PCM array computes $C_{out}$ channels of one output feature map pixel from a complete input volume of $C_{in}\times K\times K$ pixels in a single operation (that we call \textit{job}), where $C_{in}$, $C_{out}$ indicate the number of input and output channels, respectively, and $K$ is the filter size.

% Configuration of the IMA and programming of the regs
The configuration sequence of the IMA starts when a core acquires a lock over the accelerator by reading a special \textsc{acquire} register through the control interface. After that, the core can interact with the IMA by: programming the PCM devices with the weights of one or multiple layers; reading the conductance value of a PCM device; configuring a \textit{job} by setting the address of input and output data in TCDM and the ADC configuration. When the configuration is over, the execution can be started by writing to a special \textsc{trigger} register. To minimize the IMA configuration and synchronization overhead, multiple jobs can be pipelined by setting the register file with the correct strides. In this way, a whole layer can be executed with only one configuration phase.


% Two exec. models: sequential and pipelined 
We propose two execution models for back-to-back job operations of the IMA: a simpler one, sequential, and a more optimized pipelined execution model. The relative timelines are shown in Fig.~\ref{fig:ima_map_plus_timeline}. The sequential model splits the execution of the single job into three phases operated sequentially. \textsc{stream-in}: fetch data from the TCDM that is then streamed to the engine's internal DACs buffers; \textsc{computation}: analog computation on the crossbar and writing of the ADCs buffers; \textsc{stream-out}: stream data from buffers back to the TCDM. 
In Section\ref{sec:IMC_Accelerator_Performance}, we study how this model quickly becomes a bottleneck for the IMA's peak performance.

% Pipeline
In the pipelined execution model, the three aforementioned phases of different jobs can overlap each other at the cost of additional hardware resources: we add two pipeline registers before and after the DACs and ADCs buffers and we extend the \textit{Engine} FSM with additional states to control the overlapping phases: during the computing phase of the $i-th$ job (if not the last one to compute), the \textit{engine} FSM sets the streamer to start a new memory transaction to fetch the inputs for the successive $(i+1)-th$ job. When such stream-in phase has finished, if there are the results of the previous job $(i-1)-th$ to stream-out, the \textit{engine} FSM can configure the stream, as shown in Fig.~\ref{fig:ima_map_plus_timeline}. If we consider only the digital logic of the accelerator around the IMA, the pipelined approach increases the area by about 40\%, due to the doubled number of input/output registers needed to enable the pipeline. However, this overhead reduces to 5\% if we consider the total area of the accelerator (digital logic and analog IMC cross-bar), compared to the sequential approach. 

% Explanation of the pipeline
% Before starting the computation, the single-cycle \textsc{push} state move forward the pipeline, pushing the data from the input pipeline registers to the DAC buffers and from the ADC buffers to the output pipeline registers. During the computation of the $i-th$ job (if not the last one to compute), the \textit{engine} FSM enters the \textsc{comp. st.-in} state and sets the streamer to start streaming in the inputs for the successive $(i+1)-th$ job . When the stream-in phase has finished, if there are the results of the previous job to stream-out, the \textit{engine} FSM enters the \textsc{comp. st.-out} state to configure the stream. As a design choice, the stream-in phase always has highest priority over the stream-out, without impacting the execution performance. As soon as the current computation finishes ($i-th$ job), a new \textsc{push} cycle refreshes the pipeline moving the data forward. If we consider only the digital logic of the IMA, the pipelined approach increases the area by about 40\%, due to the doubled number of input/output registers. However, this overhead reduces to 5\% if we consider the total area of the accelerator (digital logic and analog IMC cross-bar), with respect to the implementation of the sequential approach. 
 

% ancillary contribution to reduce power. Consider whether to remove it or not


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DW ACCELERATOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dedicated Depth-Wise Digital Accelerator}
\label{sec:dw_accelerator_archi}

% Depth-wise accelerator architecture
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/DW_architecture_v1.pdf}
    \caption{Architecture overview of the Depth-wise digital accelerator. (a) Main overview of the accelerator, enclosed in the HWPE. (b) Execution flow of the depth-wise operation.}
    \label{fig:dw_archi}
\end{figure}


% Why we design a custom accelerator for the depth-wise
Depth-wise (DW) convolutions have been introduced in SoA DNNs such as MobileNetV2 to shrink the model size of the neural networks ( by 7 to 10$\times$) and their computational cost, with negligible accuracy drop~\cite{DBLP}. Due to their lower connectivity compared to standard convolutions (each output channel depends only on a single corresponding input channel), DW layers are generally inefficient to map on IMC arrays, as we show in section \ref{sec:IMC_Accelerator_Performance} on the \textit{Bottleneck} use-case. Moreover, a pure software execution of such kernels easily becomes a performance bottleneck for computation~\cite{ottavi2021end}. To speed up the execution of the depth-wise layers, we therefore designed a specialized digital accelerator and integrated it into the heterogeneous cluster.

% Brief description of the features of the accelerator
The accelerator we propose in this work is capable of processing depth-wise kernels on 8-bit signed input tensors and weights, accumulating the results in intermediate 32-bit registers and performing non-linear activation functions such as ReLU plus a set of ancillary functions (i.e. shifting and clipping) to bring back the final result into the 8-bit precision.
%
Fig.~\ref{fig:dw_archi} shows the general architecture of the proposed accelerator, enclosed in the dedicated HWPE interface.
% 
%THE CONTROLLER
% The \textit{Controller} contains two sets of registers: the \textit{job-dependent} ones, which normally change between multiple-jobs execution, are used to configure the pointers to access the input tensors and the weights in the TCDM memory, and the address to store the output feature map. Additional \textit{generic} registers store parameters that are static between the execution of multiple jobs, related to ReLu, clipping and shifting options. %In the current design, we focus on the 3$\times$3 depth-wise convolution, supporting stride 1the main limitation is that it is not possible to configure the stride and the size of the window filter, which are hardwired inside the engine to stride 1 and 3$\times$3 filters, respectively. 
% 
% 
% Depth-wise accelerator architecture
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/dw_loops_pipeline.pdf} % replace with PDF asap
    \caption{(a) Pseudo-Python code describing the operation of the depth-wise accelerator datapath. (b) Detail of the \textit{LD - MAC - ST} pipeline.}
    \label{fig:DW_loops_pipeline}
\end{figure}

% THE ENGINE
The depth-wise accelerator employs a weight-stationary data flow and targets 3x3 depth-wise layers -- the ones most commonly encountered in DNNs.
The weights from 16 different filters, assumed to be 8-bit signed elements, are loaded from the TCDM memory at the beginning of the computation, sign-extended, and stored into a \textit{weight buffer} that features 3x3x16 registers. 
The weights reside in the buffer until they have been used over the full input image.
% 
Input tensors are scanned by the accelerator using a vertically sliding window on the spatial dimensions, considering in each iteration 16 channels data stored in HWC layout (i.e., the same layout used by the IMA).
The vertically sliding window is implemented utilizing a \textit{window buffer} of 4x3x16 8-bit registers: 3 rows to host the current window, plus 1 row of inputs being loaded concurrently with the current window computation.
Other than the two buffers, the data path of the accelerator consists of a network of Multiply-and-Accumulate (MAC), and ancillary blocks to compute ReLu, shifting and clipping operations, as shown in Fig.~\ref{fig:dw_archi}.
%  
The MAC unit consists of 36 multipliers and a reduction tree that operate on a 3$\times$3$\times$4 block of the window buffer, passed through the ReLu and shifting\&clipping blocks, and stored in an \textit{output buffer}.
% to bring back the results into an 8-bit range. The flow is repeated four times, to consume all the input buffer. Once the execution is completed all the 16 output channels are stored in the memory through a stream request.

Fig.~\ref{fig:DW_loops_pipeline}a shows the details of the depth-wise accelerator datapath operation in the form of Python-like pseudocode.
For a given block of 16 channels, the operation starts by preloading weights.
At the start of each output column, the window buffer is loaded with the content of the first 3x3 window; then, the operation of the datapath is organized in three pipelined stages, active over an inner loop of 4 cycles as shown in Fig.~\ref{fig:DW_loops_pipeline}a and Fig.~\ref{fig:DW_loops_pipeline}b.
In the first three cycles of the inner loop, the \textit{LD} stage is active: one input pixel across 16 channels is loaded to fill the fourth row of the window buffer.
The \textit{MAC} stage is active in all cycles of the inner loop, working on 4 channels at a time.
Finally, the \textit{ST} stage is active only in the fourth cycle: during this stage, the content of the output buffer produced in the previous three cycles and the current one is streamed out of the datapath, and the window buffer slides one pixel down.
In this way, during the main body of the computation, the accelerator fully exploits the available memory bandwidth of 16 Bytes per cycle and the HWC layout of data, which is advantageous because it is the same layout used by the IMA.
Overall, the execution of a depth-wise layer on the dedicated accelerator improves by 26$\times$ over a pure software implementation, achieving an average performance of 29.7 MAC/cycle.
% The to exploit the HWC layout of data and the available memory bandwidth of 16 Bytes per cycle, 
% Computing paradigm and the pipelined approach
% To reduce the latency of the execution, the DW Accelerator supports pipelined jobs but also pipelined intra-job computing phases.
% During the MAC evaluation phase, the window buffer is allowed to request new streams to fill the additional row in the buffer, overlapping the streams to the computing phase. At the next MAC evaluation, the window to be convolved with the filters is obtained shifting by one row down the previous window and reusing two lines of it, increasing the data reuse rate. Such a mechanism is performed until the scan operation reaches one spatial edge of the image.
% In this case, a \textit{clear} operation on the entire window buffer is needed. Despite the penalty of fetching the whole window from the memory whenever an edge of the input image is reached, we measure that our approach reduces the memory accesses by more than 60\% (e.g. simple estimates on a 28$\times$28 image would result in 65\% of memory access savings with the discussed approach). 

% conclusive sentence of the pipeline (dynamic mux)
%To reduce the execution cycles, also the output streams can overlap the execution phase or the stream-in phase. In this case, the dynamic multiplexer (that muxes the two streams) handles the eventual concurrent access to the master port of the data interface towards the TCDM through a round-robin arbitration mechanism. From an empiric evaluation on the layers benchmarked in this work, no stalls or loss of performance are observed with the presented dynamic approach.

% % MAC Units
% The MAC unit consists of 36 multipliers and a reduction tree that operate on a 3$\times$3$\times$4 block of the input buffer at a time, producing 4 intermediate results per cycle, stored into 32bit registers. The results are then passed through the ReLu and shifting\&clipping blocks to bring back the results into an 8-bit range. The flow is repeated four times, to consume all the input buffer. Once the execution is completed all the 16 output channels are stored in the memory through a stream request. 



==> text/05_results_and_discussion.tex <==
%%% RESULTS SECTION
\section{Experimental Results}
\label{sec:Experimental_Results}
% Introduction to the section
In this section we evaluate the proposed heterogeneous cluster from a physical viewpoint, measuring and discussing power, area, and timing costs of the analog/digital system and from a performance and energy efficiency viewpoint, benchmarking DNN layers such as point-wise, depth-wise, and \textit{Bottleneck} layers, representative of modern neural networks widely used in edge AI classification tasks.

% TABLE: physical characterization of the IMA
% Floorplan
\label{sec:Physical_Implementation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{images/Floorplan.pdf}
    \caption{(a) Placed and Routed design of the heterogeneous cluster. (b) Area breakdown of the system.}
    \label{fig:floorplan}
\end{figure*}
%\input{text/Physical_table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PHYSICAL IMPLEMENTATION SETUP AND EARLY RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Physical Implementation}
% Implementation. Corners, how we integrate ima numbers, comments on area and timing results
To characterize the system in terms of area, power, and performance, we implement the cluster using the GlobalFoundries 22nm FDX technology node. We synthesize the heterogeneous cluster with Synopsys Design Compiler-2019.12 and we perform a full place\&route flow using Cadence Innovus 20.12, targeting the worst-case corner (SS, 0.72V, -40°/125°). The floorplan of the system is reported in Fig.~\ref{fig:floorplan}. The analog IMC accelerator models, validated on silicon and modeled through silicon characterization of 14 nm prototypes, are fed into technology libraries (\textit{.lef}, \textit{.db}, and \textit{.lib}) integrated into the front-end and back-end flows of the system. The area, the timing, and the power consumption of the IMC accelerator are extrapolated from the on-chip measurements reported in~\cite{hermesCor}, properly scaled to the 22nm technology node. The power scaling is done according to the classical scaling theory under constant frequency, scaling power by $a\cdot b ^2$, where $a$ denotes the dimensional scaling and $b$ is the voltage scaling factor. The area scaling follows the dimensional scaling. We assume that the IMA latency will remain constant. The total area of the heterogeneous cluster is 2.5 $mm^2$, partitioned among the several hardware blocks as shown in Fig.~\ref{fig:floorplan}(b). As expected, the IMA sub-system and the 512 kB of TCDM memory occupy the major part of the total area ($\sim$1/3 IMA, $\sim$1/3 TCDM, 1/3 the rest of the cluster), while the depth-wise accelerator has a negligible impact (2.1 \%). The maximum operating frequency achievable by the final design is 500 MHz.

% power measurements methodology with IMA power summary
To perform the power measurements we run parasitics-annotated gate-level netlist simulations of the digital part of the system in the typical corner (TT, 25C) at the operating voltage of 0.8V, executing the DNN layers introduced above. The VCD traces of the simulations are then analyzed with the Synopsys PrimeTime tool. The extracted power is then integrated with the power extrapolated for the IMC accelerator~\cite{hermesCor}.
%
%Table~\ref{tab:IMA_numbers} reports a summary of the physical implementation results of the heterogeneous cluster. 
% Final remark on the methodology
Hence, all the results that we present in this section and the following ones include the overheads (i.e. timing, area, power) caused by the clock tree implementation, accurate parasitic models extraction, cell sizing for setup fixing, and delay buffers for hold fixing.
We emphasize that neglecting these factors would cause significant underestimations in the clock tree dynamic power.

% IMA ROOFLINE IMAGE
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{images/Roofline.pdf}
    \caption{Roofline model of the IMA heterogeneous system. The compute roof of the IMA is a diagonal line, which depends quadratically on the operation intensity, not on the cluster frequency. The intersection of a bandwidth line with the compute roof defines a region where the performance points can lay for that configuration. In (a) and (b) cluster is running at 500MHz and 250MHz, respectively, with sequential execution of IMA.  In (c) it runs at 250 MHz with a pipelined execution model for the IMA.}
    \label{fig:roofline}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% IMA PEAK PERFORMANCE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IMC Accelerator Performance}
\label{sec:IMC_Accelerator_Performance}
% limitations to the IMA peak performance
First, we analyze the peak performance achievable by the IMA. An important point to stress is that, in contrast with digital accelerators, the maximum performance of the IMC array is only related to its MVM operation latency and its size (256$\times$256 in the context of this work). The peak throughput is 1.008 TOPS, given by the maximum number of operations (256 $\times$ 256 $\times$ 2 OPs) that can be executed in its latency of 130ns~\cite{hermesCor}. In practice though, the real throughput achievable is typically scaled by the utilization factor of the array: only if we map a 256 output-channel / 256 input-channel point-wise layer we can achieve the maximum utilization rate and, thus, throughput.
%This reasoning is highlighted in the plots in Fig.~\ref{fig:roofline}, where the compute roof of the IMA is a diagonal line and not a line parallel to the x-axis, as is typically the case for digital systems.
Another factor that limits the real performance of the IMA sub-system is the memory bandwidth that the heterogeneous cluster can sustain to feed the IMA with new input data and to store the IMA results into the TCDM memory. If the computation is too fast compared to the stream-in and stream-out time, we lose performance because we are limited by the bandwidth of the system. 

% PULP cluster potentially offers high bandwidth. Explorations carried out
The PULP cluster can potentially offer high memory bandwidth towards the L1 memory thanks to the tightly-coupled interconnect scheme, at the cost of an increased interconnect area (which scales linearly with the bit-width of the system bus), power, and timing. 
% Dimension the system-bus to sustain IMA computation
To find the width of the system bus able to sustain the IO requirements of the IMA at the lowest area overhead, we benchmark synthetic point-wise layers with different utilization rates of the IMC array (from 5\% to 100\%), varying the width of the IMA sub-system bus from 32-bit up to 512-bit.
%To find the optimal width of the system bus able to sustain the bandwidth requirements of the IMA, we benchmark synthetic point-wise layers with different utilization rates of the IMC array (from 6\% to 100\%), varying the width of the IMA sub-system bus (and the number of master ports of the logarithmic interconnect) from 32bits up to 512bits (i.e. from 1 to 16 master ports).

% Two points investigated: 500 MHz and 250 MHz -- pipelined and non-pipelined execution model. explanation of compute roof of IMA
In Fig.~\ref{fig:roofline} we report the outcomes of our exploration as a roof-line plot~\cite{williams2009roofline}. The computing latency of the IMA does not depend on the cluster frequency, leading to two considerations: first, the compute roof of the IMA is a diagonal line proportional to the operation intensity (in other words, to the utilization factor of the IMA cross-bar) and not a line parallel to the x-axis, as is typically the case for digital systems; second, since the IMA computing latency is fixed, its memory bandwidth requirement change as we reduce or increase the cluster clock frequency. We investigate two operating frequencies, the maximum achievable one by the system when operating at high-voltage (500 MHz at 0.8V) and the maximum one achievable at low-voltage (250 MHz at 0.65V), and we compare the sequential and the pipelined execution models of the IMA. %The intersection of a bandwidth line with the compute roof in Fig.~\ref{fig:roofline}, defines a region where the performance points can lay for that configuration. If the performance points are close to the bandwidth border, this means that we are memory bound; on the contrary, we are compute bound. A bandwidth line that never intercepts the compute roof means that the considered bandwidth overcomes the requirements of the IMC accelerator.

% Comment roofline at 500 MHZ, under-utilization of the bandwidth, explain why
%In the Fig.~\ref{fig:roofline}.(a) the cluster is running at 500 MHz and we adopt the sequential execution model for the IMA. We observe that only the blu line, corresponding to the bandwidth generated by a 32bit wide bus, intercepts the compute roof; in all the other cases the performance is never limited by the system bandwidth: two master ports (i.e. 64b wide bus) are sufficient to fulfill the computing requirements of the IMA. However, analyzing the performance at any of the system-bus configurations above 32bits we notice a gap between the compute roof and the real throughput, suggesting that we are under-utilizing the bandwidth of the system. The reason is that in the sequential model, as discussed in Section \ref{sec:ima_description}, 8\% to 40\% (depending on the size of the layer considered) of the total execution cycles are spent in stream-in and stream-out phases. In the rest of the execution, when the IMA is in the computing phase, the system bus is not solicited.
% V2
In Fig.~\ref{fig:roofline}(a) the cluster is running at 500 MHz and we adopt the sequential execution model for the IMA. We observe that only with a 32-bit wide bus we are memory bound and a 64-bit wide data interface of the IMA subsystem is sufficient to fulfill the computing and IO requirements of the IMA. However, analyzing the performance at any of the system bus configurations above 32-bit we notice a gap between the compute roof and the real throughput, suggesting that we are under-utilizing the bandwidth of the system. The reason is that in the sequential model, as discussed in Section \ref{sec:ima_description}, 8\% to 40\% (depending on the size of the layer considered) of the total execution cycles are spent in stream-in and stream-out phases. In the rest of the execution, when the IMA is in the computing phase, the system bus is not solicited.


% Comment roofline at 250 MHz
%With the same bus width, the lower the frequency the lower the bandwidth at disposal of the analog accelerator. Hence, at 250 MHz we observe that higher bus-width (i.e. 128bits) is necessary to preserve the peak performance of the IMA, as depicted in Fig.\ref{fig:roofline}.(b). However, also in this case we are quite far from reaching the computing roof of the IMA with the sequential execution model of the IMA.
% V2
Analyzing the scenario where the cluster runs at 250 MHz we observe that higher bus-width (i.e. 128-bit) is necessary to preserve the peak performance of the IMA, as depicted in Fig.\ref{fig:roofline}(b). However, also in this case the sequential execution model is quite far from reaching the computing roof of the IMA.
% 
% Comment the roofline with the pipelined IMA
%Despite the unavoidable area overhead with respect to the sequential execution model (which, however, is limited to 5\% if we consider the whole IMA sub-system, including the analog macro), Fig.\ref{fig:roofline}.(c) shows that the pipelined solution guarantees the best performance. At the system-level the optimal configuration is with a 128b-wide system-bus: from Fig.\ref{fig:roofline}.(c) we notice that with 32b-/64b-wide system-bus configurations we are memory bound, above the 128b-wide system-bus there is no improvement in the computation as we reach the compute roof. In this configuration, we achieve a peak of 958 GOPS at 250 MHz, only 10\% less than the performance at the compute roof. That 10\% is the programming overhead, necessary to configure the accelerator and start the execution.
%
Despite the unavoidable area overhead compared to the sequential execution model (which, however, is limited to 5\% if we consider the whole IMA sub-system, including the analog macro), Fig.\ref{fig:roofline}(c) shows that the pipelined solution guarantees full utilization of the bandwidth. At the system level, the optimal configuration is with a 128-bit wide system bus: using a narrower system bus, throughput is memory-bound, while using a wider one, performance does not improve, as computation is in a  compute-bound region. In the optimal system configuration, the IMA can achieve a peak of 958 GOPS at 250 MHz, only 10\% less than the theoretical peak performance at the compute roof, due to the programming overhead necessary to configure the accelerator and start the execution.


% Removed because it is reduntant ---> We are overlapping the stream-in and stream-out phases with the computation itself, and also when the IMA is in the compute state, the system-bus is working to stream-in inputs of the successive jobs or to stream-out the results of previous jobs, resulting in a more balanced exploitation of the system capabilities. 
%% BOTTLENECK RESULTS (perf, en. efficiency, area efficiency)
\begin{figure*}[t]
\centerline{\includegraphics[width=0.85\textwidth]{images/perf_EE_areaE.pdf}}
\caption{(a) Performance (in GOPS), (b) Energy Efficiency (in TOPS/W), and (c) Area Utilization Efficiency (in GOPS/$mm^2$) of the \textit{Bottleneck} layer running on the cluster at 500 MHz with 128-bit wide system-bus. The area efficiency is related to the effective area of the PCM arrays utilized to implement the \textit{Bottleneck} (including padding necessary to map the depth-wise on the IMA).}
\label{fig:res_compressed}
\end{figure*}

%In \textsc{ima+dw} the depth-wise layer is offloaded to the digital accelerator, in \textsc{ima $c_{job16}$} and \textsc{ima $c_{job8}$} it is offloaded to the IMA with two different HW configurations, in \textsc{hybrid} it is offloaded to the cores. The residual connections are always run on the cores, the point-wise layers are always offloaded to the IMA, except for the \textsc{cores} case, where all the layers are computed by the cluster's cores. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BOTTLENECK LAYER RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Case Study: The \textit{Bottleneck} Layer}
\label{sec:The_Bottleneck_Layer}
\label{sec:ima_depthwise}
\label{sec:bottlenecs_res}

% BOTTLENECK LAYER ON IMA
\begin{figure}[t!]
\centerline{\includegraphics[width=0.85\linewidth]{images/old_paper/memory_mapping_ima_2.png}}
\caption{Components of MobilenetV2 \textit{Bottleneck} block with stride = 1 and mapping structure in the PCM crossbar for depthwise layers. All the gray rectangles are padding required for computing more than 1 channel per job.}
\label{fig:bottleneck}
\end{figure}



% brief introduction
To highlight the advantages, the trade-off, and the challenges of IMC on realistic use cases for edge computing and to assess the benefits of the presented heterogeneous system, we benchmark the \textit{Bottleneck} layer of a MobileNetV2 DNN. We analyze three different computation mappings that are possible on the analog/digital system, compared to the baseline, which executes all the layers of the \textit{Bottleneck} on the software cores using optimized software libraries~\cite{garofalo2020pulp}.
%a pervasive model in many edge computing AI-enhanced classification and recognition tasks.
% params of bottleneck layer, justify the selected layer
The parameters of the selected \textit{Bottleneck} layer are reported in Fig. \ref{fig:bottleneck}: this configuration is chosen so that all the weights and activations fit the on-cluster TCDM (512 kB), without requiring any activation data tiling~\cite{burrello2020dory}, the in-depth study of which is beyond the scope of this work.
% introduce the three possible execution flows
%To validate the solution that achieves the best performance and the efficiency, we propose and compare three different execution flows of the bottleneck layer which are possible on the proposed heterogeneous systems, described below.

% first execution flow: all on IMA using IM2COL approach. Point-wise efficient to map on IMA
The first possible execution mapping is to offload all the layers of the \textit{Bottleneck} to the IMA accelerator, except  for the residual connection, which is always offloaded to the cluster's cores. To map the weights of the layers on the IMC cross-bar, we adopt the \textsc{im2col} approach~\cite{garofalo2020pulp}. Mapping point-wise layers is straightforward: each $1 \times 1 \times C_{in}$ filter is mapped across the height of the cross-bar (one column), more filters are mapped across the columns. If the layer parameters did not fit the size of the array, we would have to split the weights over multiple IMAs. We postpone the analysis of more complex scenarios, such as these, to Section~\ref{sec:discussion} and we focus on the baseline case of a fully fitting layer here.

% Depth-wise inefficient to map on IMA
Contrarily to the point-wise layer, the depth-wise one is very inefficient to map on the IMA cross-bar. In depth-wise convolutions, each output channel depends only on the corresponding input channel: to make them suitable for mapping on the cross-bar array, a $K \times K$ kernel with $C$ in/out channels must be expanded into a dense form, with all the weights out of a diagonal set to zero (padding), as shown in Fig.~\ref{fig:bottleneck}. Assuming a hypothetical IMC array large enough to fit all the weights and padding of the layer, out of $K^2 \times C^2$ crossbar locations programmed with weights or zeros, only $K^2\times C$ of them would concur to the kernel computation.%, resulting in low utilization of the cross-bar. 

% Strategy to reduce useless occupancy of the crossbar cells
% ==== V2 ====
To reduce the useless occupancy of crossbar cells (i.e. programmed with zeros), a different approach is to split the computation of $C_{out}$ pixels, that normally would be computed in a single operation (what we call \textit{job}), over multiple jobs, each of which computes  $C_{job}<C_{out}$ pixels. As a trade-off, this leads to a smaller amount of operations per job, reducing the overall performance. The advantage of this method is that the total number of crossbar elements required to map the depth-wise kernel is $N_{xbar} = K^2 \times C \times C_{job}$, reducing the number of the overall programmed cells (with zeros and weights) by a factor of $C_{out} / C_{job}$ compared to the previous approach, at the cost of additional $N_{jobs}=C_{out}/ C_{job}$ jobs per output pixel to complete the execution of the kernel (note that in the previous case 1 job per $C_{out}$ pixels is possible only on ideal infinite sized cross-bar).
% ==== V1 ====
%To reduce the useless occupancy of crossbar cells (i.e. programmed with zeros), a different approach is to split the execution of the depth-wise in separate jobs. As a trade-off this leads to a smaller amount of operations per job, reducing the overall performance. However, the total number of crossbar elements required to map the depth-wise kernel is $N_{xbar} = K^2 \times C \times C_{job}$, where $C_{job}$ is the number of output channels per job and can be sized at design-time. This strategy reduces the number of the overall programmed cells (with zeros and weights) by a factor of $C / C_{job}$, at the cost of additional $N_{jobs}=C / C_{job}$ jobs to complete the execution of the kernel (note that in the previous case 1 job is enough to complete the execution only on ideal infinite sized cross-bar).

% Real-sized IMA and mapping challenges of considered depth-wise
Mapping all the layers of the targeted \textit{Bottleneck} following the first approach is not feasible on the 256$\times$256 cross-bar array we use: we would require 23$\times$ more cross-bar locations than the real number of weights, running out of IMC resources. Hence, we analyze the costs of separating the depth-wise in multiple jobs, considering two parameters: $C_{job} = 8$ and $C_{job} = 16$, which translates to an increase of 25\% and 54\% in the number of devices, respectively. Empirically, we consider these configurations as a reasonable trade-off between performance and occupancy of the cross-bar. The two configurations are referred to as \textsc{ima $c_{job8}$} and \textsc{ima $c_{job16}$}, respectively.
%Despite the depth-wise weights account only for $\sim$4\% of the total weights, if we map the targeted Bottleneck on the 256$\times$256 cross-bar array we use in this work, we would require 23$\times$ more cross-bar locations than the real number of parameters, because of the padding necessary in the depth-wise layer, running out the IMC crossbar locations available. This confirms that the first mapping option is not viable in practical cases. Hence, in this work we tackle the problem of mapping the depth-wise kernels by separating the depth-wise in multiple jobs, considering two parameters: $C_{job} = 8$ and $C_{job} = 16$, which translates to an increase of 25\% and 54\% in the number of devices respectively. Empirically, we consider these configurations as a reasonable trade-off between performance and occupancy of the cross-bar. The results of this solution are reported in Fig.~\ref{fig:res_compressed} with the two configurations referred to as \textsc{ima $c_{job8}$} and \textsc{ima $c_{job16}$} respectively,


% Second execution flow: point-wise on IMA, rest on the cores
The second mapping we analyze executes the point-wise layers on the IMA and the depth-wise kernels on the 8 RISC-V cores of the cluster. The software kernels for the depth-wise are derived from an optimized parallel software library tailored on PULP-based clusters~\cite{garofalo2020pulp}. Since such kernels require the input data to be in Channel-Height-Width (CHW) layout and since the output from the point-wise layer (from the IMA) is in Height-Width-Channel (HWC) layout, additional execution cycles are needed for on-the-fly data marshaling operations. The output is generated in the HWC format instead and can be forwarded to the IMA with no additional overhead. This configuration is referred to as \textsc{hybrid} and requires the storage of depth-wise weights in the TCDM, instead of in the IMA crossbar. This is a reasonable trade-off since the depth-wise weights usually account for no more than 10\% of the total of a depth-wise based neural network~\cite{sandler2018mobilenetv2} ($\sim4\%$ in the considered \textit{Bottleneck} layer). 

% Third execution flow: point-wise on IMA, depth-wise on digital accelerator, rest on cores
The third mapping solution, indicated as \textsc{ima+dw}, runs the point-wise layers on the IMA, the depth-wise layers on the dedicated digital accelerator, and the residual layer on the cores. The digital accelerator accepts input data and weights in HWC format and produces outputs in HWC format, requiring no additional data marshaling operations during the \textit{Bottleneck} layer execution. 
%

Benchmarking results are provided in Fig.~\ref{fig:res_compressed} for all the solutions discussed above, in terms of performance, energy efficiency, and area utilization efficiency. The width of the system bus is 128-bit and we adopt the pipelined execution model for the IMA; as demonstrated in Sec.~\ref{sec:IMC_Accelerator_Performance}, this configuration maximizes performance. The cluster operates at 500 MHz at 0.8V, in typical operating conditions (TT, 0.8V, 25C). 

% Performance comments
We can notice that despite a significant area utilization of the IMC array, the performance of \textsc{ima $c_{job16}$} and \textsc{ima $c_{job8}$} are only 2.27$\times$ and 1.23$\times$ higher than a pure software execution of the \textit{Bottleneck}. Efficiency is even worse: 1.23$\times$ lower energy efficiency and the same area efficiency of \textsc{ima $c_{job8}$}, and comparable energy and area efficiency of \textsc{ima $c_{job16}$} compared to the \textsc{cores} demonstrate that IMC arrays are not efficient to host sparse layers like the depth-wise. 
%
The \textsc{hybrid} solution instead achieves 4.6$\times$ better performance and 3.4$\times$ better energy efficiency than the \textsc{cores} configuration. Despite software-based execution of depth-wise layers, this solution overcomes the $c_{job16}$ configuration by 2$\times$ in terms of performance, by 2.3$\times$ in terms of energy efficiency, and by 2.1$\times$ in terms of area efficiency. The peak performance is achieved in the \textsc{ima+dw} configuration, improving by 2.6$\times$ and 11.5$\times$ over the \textsc{hybrid} and \textsc{cores} solutions, respectively. By offloading point-wise layers to the IMA and depth-wise layers to the dedicated digital accelerator, we fully exploit the potential of the two hardware blocks, while the cores handle their configuration, the workload dispatching, and ancillary aggregation operations, such as the residual connection. This synergistic approach, enabled by the fact that cores, IMA, and depth-wise accelerator all share the same memory at L1, stands out also as the most efficient one, overcoming 2.7$\times$ and 9.2$\times$ the \textsc{hybrid} and \textsc{cores} configurations, in terms of energy efficiency, and by 2.5$\times$ and 10.2$\times$ the same configurations in terms of area efficiency.

% COMMENTS ON AREA EFFICIENCY
%To put in perspective the cost of increasing the throughput using IMA, the area efficiency reported in Fig~\ref{fig:res_compressed}(c) is related to the effective area of the PCM arrays utilized to implement the Bottleneck (including padding necessary to map the depth-wise on the IMA). The \textsc{ima+dw} solution has the best result requiring 5.42$\times$ and 10$\times$ smaller PCM area for the same bottleneck when compared to \textsc{ima $c_{job16}$} and \textsc{ima $c_{job8}$}, respectively. Considering also the area of the cluster itself (\textsc{cores}), we obtain 10.2$\times$ better GOPS/$mm^2$.

\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{images/exec_cycles.pdf}
\caption{Normalized Performance, compared to full software implementation (\textsc{cores}), of point-wise (left) and \textit{Bottleneck} (right) layers. For the right-side analysis, the impact of each layer on the execution of the whole Bottleneck is shown, considering the different computing mapping solutions enabled by the heterogeneous cluster.}
\label{fig:totCycles}
\end{figure}

% FINAL REMARK
Fig.~\ref{fig:totCycles} shows the execution breakdown of the \textit{Bottleneck} layer. In a pure software execution scenario, the point-wise layers dominate the computation (\textsc{cores}). The IMA shows significant acceleration in such dense MVM-based operations (left-sided Fig.~\ref{fig:totCycles}), moving the performance bottleneck on other layers like the depth-wise. However, the IMA itself is not capable of mitigating this Amdahl's effect, since the execution of the depth-wise on the IMA is not efficient and dominates the total execution cycles (\textsc{ima $c_{job8}$} and \textsc{ima $c_{job16}$}). Execution of depth-wise convolutions on the cores (\textsc{hybrid}) improves execution time, but this block remains by far the slowest one. On the other hand, offloading the depth-wise layer to the digital accelerator (\textsc{ima+dw}) eliminates the performance bottleneck as the execution time of the depth-wise layer is comparable to the other components of the \textit{Bottleneck}, such as point-wise layers and residuals.




==> text/07_SOA_Comparison.tex <==
\input{text/Soa_table_v2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COMPARISON WITH THE SOTA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comparison with the State-of-the-Art}
\label{sec:comparison_with_soa}

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/final_plot.pdf}
    \caption{Performance of the MobileNetV2, normalized on the compute roof of the each considered IMC-based computing model. On the \textsc{ima+asic} is not possible to deploy the network model, due to architectural limitations.}
    \label{fig:final_plot}
\end{figure}

Tab.~\ref{tab:SOA_TABLE} reports the comparison of our scaled-up system with state-of-the-art solutions. Both fully digital and mixed-signal solutions are considered.
%Tab.~\ref{tab:SOA_TABLE} reports the comparison of our scaled-up system with state-of-the-art solutions in terms of area, peak efficiency, performance and further metrics related specifically to machine learning workload. Both fully digital and mixed-signal solutions are considered.

% ARCHITECTURE
In terms of architectural capabilities, the paradigm we propose is superior compared to the others, as it provides full hardware support for a  wide range of workloads and integer precisions both in the analog and digital domain, enabling de facto efficient end-to-end execution of complex neural network models such as the MobileNetV2. On one hand, Vega \cite{rossi2021vega} is an architecture similar to ours, with 9 RISC-V cores integrated into a parallel cluster, but it does not include analog IMC cores, nor dedicated accelerators for depth-wise. On the other hand, the architecture in \cite{jia2020programmable} features only a tiny 32bit RISC-V processor and a charge-based IMC array, but integrated into the system through a loosely-coupled scheme, directly connected to the 32b AXI bus. The loosely-coupled integration of the IMA forms a huge performance bottleneck even for standard convolutions (as shown in section \ref{sec:IMC_Accelerator_Performance}). In the end, authors of \cite{zhou2021analognets} extend a PCM-based IMC array with a digital fixed data-path that performs only activation and pooling operations, while a small SRAM memory acts as a layer-to-layer intermediate buffer.

% PEAK PERFORMANCE AND EFFICIENCY
In terms of peak performance and efficiency, our solution is comparable with others. Jia \textit{et al.} \cite{jia2020programmable} show a peak of 2.19 TOPS and 400 TOPS/W on 1b-1b MVM with IMA, both higher than what we show. However, it should be noted that these numbers scale with the bit-precision of the input-vectors and the matrix elements, resulting comparable with out peak in 8b-4b MVMs. With respect to \cite{zhou2021analognets}, our solution shows lower peak performance and efficiency. Being the in-memory macro the same, such a results only comes from the bigger sized array they use (1024$\times$512 compared to 256$\times$256), while a loss as little as 10\% of the peak is attributable to the integration of the IMA into a complex system like the one we propose, as we show in Section \ref{sec:bottlenecs_res}. With respect to Vega, which is a fully digital solution, we are better by 31$\times$ in terms of performance, with 4.92$\times$ higher energy efficiency.

% COMPARISON ON MBV2 INFERENCE
%In the end, we compare our solution with other IMC approaches, on the end-to-end execution of the MobileNetV2. As shown in %Fig.~\ref{fig:final_plot}, we compare
%In the end, we compare our architectural paradigm on the end-to-end execution of the MobileNetV2 with other IMC approaches. In reference to Fig.~\ref{fig:final_plot} we compare different computing models: IMA extended with digital ASICs, IMA extended with 
In the end, we compare our architectural paradigm on the end-to-end execution of the MobileNetV2. Despite the architecture presented in \cite{jia2020programmable} has been demonstrated on a 9 CNN layers NN, it could potentially run the MobileNetV2. Though, the only execution flow that this architecture allows is to offload the point-wise layers to the IMC array and the depth-wise and residual layers to the tiny RISC-V processor. We estimate the execution latency of the MobileNetV2 point-wise layers from the peak performance that the IMC array achieves on 8b-4b MVM operations (scaled from 1b-1b MVMs performance as explained in \cite{jia2020programmable}). The latency of 8b-8b depth-wise convolutions is estimated from the results we obtain benchmarking the depth-wise layers on our cluster's cores, properly scaled considering that: our core is $\sim$10$\times$ faster on a per-core basis with respect to their tiny processor, due to the enhanced Instruction Set Architecture \cite{gautschi2017near}; if we expand the picture to the entire cluster we would look at another $\sim$7$\times$ improvement factor due to the parallelism \cite{garofalo2020pulp}. Taking this to account, our estimates show two orders of magnitude higher inference latency on this architecture compared to ours.

Due to architectural limitations, it is not possible to execute the end-to-end inference of the MobileNetV2 on the solution presented in \cite{zhou2021analognets}. First, a single IMC array can not host all the layers weights of the MobileNet. Second, there are no programmable cores to handle residual connections and control operations. With respect to the fully digital solution \cite{rossi2021vega}, we show 10$\times$ and 2.5$\times$ improvement in terms of inference latency and energy,  thanks to the In-Memory cores and the dedicated digital accelerator.

% Architecture 
%Our tightly-coupled RISC-V heterogeneous cluster is the only solution of this kind to provide hardware support for a wide range of workloads and operation precision formats in the integer domain, enabling the end-to-end execution of complex neural network models such as the MobileNetV2, not feasible on mixed-signal solutions like \cite{jia2020programmable} and \cite{zhou2021analognets}.
% comparison with verma et al.
%On one hand, the architecture in \cite{jia2020programmable} features a tiny 32bit RISC-V processor and a charge-domain IMC array integrated into the system through a loosely-coupled scheme, directly connected to the 32b AXI bus. This solution is not viable to sustain the computational requirements of modern neural network models. The loosely-coupled integration of the IMA forms a huge performance bottleneck even for standard convolutions (as shown in section \ref{sec:IMC_Accelerator_Performance}). Moreover, deploying the depth-wise layers on the tiny RISC-V core would be inefficient. Our core, which is however not our best solution for the depth-wise, is already $\sim$10$\times$ faster on a per-core basis with respect to their tiny processor. If we expand the picture to the entire cluster we would look at another $\sim$7$\times$ improvement factor due to the parallelism. Despite the chip has been demonstrated on a 9 CNN layers NN, trained on the small CIFAR-10 dataset, they show performance and efficiency that are in line with our results, resulting from a wider network benchmark. In terms of IMA performance and efficiency, they show a peak of 2.19 TOPS and 400 TOPS/W on 1b-1b MVM, both higher than our solution. However, it should be noted that these numbers scale with the bit-precision of the input-vectors and the matrix elements, resulting in the same range of our proposed solution for 8b-4b MVMs. 

%Comparison with analognets
%On the other hand, authors of \cite{zhou2021analognets} extend a PCM-based IMC array with digital logic that performs activation and pooling operations. A small SRAM memory acts as a layer-to-layer intermediate buffer. Compared to them, our solution shows lower peak performance and efficiency. Being the in-memory macro the same, such a results only comes from the bigger sized array they use (1024$\times$512 compared to 256$\times$256). The presented architecture can not host the execution of NN models that do not fit the limited size of the single IMC array, for the reasons highlighted in section \ref{fig:discussion}. Moreover, there is no dedicated support for the depth-wise convolution. To bypass the inefficiency of the depth-wise mapping on the IMA and to meet the limitations of the underlying architecture the authors replace all the depth-wise layers of the micronets with standard convolutions, building custom models called AnalogNets. Such a solution, dual with respect to our approach, is unlikely to be adopted for mainstream AI-enhanced edge applications. 

% comparison with vega
%Vega \cite{rossi2021vega} is an architecture similar to ours, with 9 RISC-V cores integrated into a parallel cluster, but it does not include analog IMC cores, nor dedicated accelerators for depth-wise. This chip has been demonstrated on the end-to-end inference of the same MobilenetV2 we benchmarked. However, we show 10$\times$ and 2.5$\times$ improvement in terms of inference latency and energy, mainly thanks to the In-Memory cores and the dedicated digital accelerator. In terms of peak integer performance, we are better than Vega by 31$\times$, with 4.92$\times$ higher energy efficiency.


% VERMA et al.
%The only execution flow that this architecture allows is to offload the point-wise layers to the IMC array and the depth-wise and residual layers to the tiny RISC-V processor. The latency of point-wise execution is estimated from the peak performance that the IMC array achieves on 8b-4b MVM operations (scaled from 1b-1b MVMs performance as explained in \cite{jia2020programmable}). The latency of 8b-8b depth-wise convolutions is estimated from benchmarking results of the cores of our heterogeneous cluster at the light of the following considerations: our core is $\sim$10$\times$ faster on a per-core basis with respect to their tiny processor, due to the enhanced Instruction Set Architecture \cite{gautschi2017near}; if we expand the picture to the entire cluster we would look at another $\sim$7$\times$ improvement factor due to the parallelism \cite{garofalo2020pulp}. Our estimates show two orders of magnitude higher inference latency on this architecture.

% ARM + IBM
%On this architecture is not possible to execute the end-to-end inference of the MobileNetV2. First, a single IMC array can not host all the layers of the MobileNet. Second, there is no hardware support for the depth-wise convolutions. Third, there is no DMA to communicate with higher memory levels. Fourth, there is not a programmable cores to handle residual connections and execution control operations. 

==> text/Physical_table.tex <==
% IMA PHYSICAL CHARACTERIZATION
\begin{table}[t]
\centering
\begin{tabular}{|lllll|}
\hline
\multicolumn{5}{|c|}{\textbf{PCM IMC array characterization }}                                                                                                                                                                                                                              \\ \hline
\multicolumn{1}{|c|}{}                                                                               & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Area {[}mm$^2${]}\end{tabular}}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Power  {[}mW{]}\end{tabular}}} \\
\multicolumn{1}{|l|}{}                                                                               & \textbf{14nm \cite{hermesCor}}                           & \multicolumn{1}{l|}{\textbf{22nm}}              & \textbf{14nm \cite{hermesCor}}                             & \textbf{22nm}                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Total}}                                                                 & \multicolumn{1}{r}{0.528}               & \multicolumn{1}{r|}{0.83}                       & \multicolumn{1}{r}{85.4}                  & \multicolumn{1}{r|}{134.2}   \\               \hline
\end{tabular}
\vspace{3mm}
\caption{Area and Power consumption of the PCM-based IMC array. Results measured on silicon prototype in 14nm and scaled to 22nm.}
\label{tab:IMA_numbers}
\end{table}

==> text/SoA_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t!]
\centering
\caption{Comparison with the State-of-the-Art.}
\vspace{3mm}
\begin{tabular}{lccclcccl}
\hline
\multicolumn{1}{l|}{}                                                                                                        & \multicolumn{2}{c|}{\textbf{VERMA et al.}}                                                                   & \multicolumn{2}{c|}{\textbf{VEGA \cite{rossi2021vega}}}                                                                       & \multicolumn{2}{c|}{\textbf{ARM+ IBM}}                                                                         & \multicolumn{2}{c}{\textbf{This Work}}                                                                                                      \\ \hline
\multicolumn{1}{l|}{\textbf{Technology}}                                                                                     & \multicolumn{2}{c|}{65 nm}                                                                                   & \multicolumn{2}{c|}{22nm}                                                                                & \multicolumn{2}{c|}{14nm}                                                                                      & \multicolumn{2}{c}{22nm}                                                                                                                    \\ \hline
\multicolumn{1}{l|}{\textbf{Architecture}}                                                                                   & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Mixed-Signal IMC,\\  Digital NMC, \\ RISC-V CPU\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}RISC-V\\ Multi-Core\\  Cluster,\\  HWCE\end{tabular}}     & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}AnalogCIM, \\  Dgital \\ Activation \\ Processing\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}RISC-V \\  Multi-Core\\  Cluster,  \\  Analog CIM,\\ Depth-wise \\ digital acc.\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Target   \\ Application\end{tabular}}}                                & \multicolumn{2}{c|}{CNN Inference}                                                                           & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}IoT AI-enhanced \\ Applications\end{tabular}}             & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}KWS and VWW \\ based on AnalogNets\end{tabular}}                & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}IoT AI-enhanced \\ Applications\end{tabular}}                                                 \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total Area   \\ {[}mm2{]}\end{tabular}}}                              & \multicolumn{2}{c|}{13.5}                                                                                    & \multicolumn{2}{c|}{12}                                                                                  & \multicolumn{2}{c|}{3.2}                                                                                       & \multicolumn{2}{c}{$\sim$30}                                                                                                                \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total \\ On-chip  \\  Memory\end{tabular}}}                           & \multicolumn{2}{c|}{72 kB}                                                                                   & \multicolumn{2}{c|}{$\sim$6MB}                                                                           & \multicolumn{2}{c|}{128 kB}                                                                                    & \multicolumn{2}{c}{512 kB}                                                                                                                  \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Processing   \\ Engine\end{tabular}}}                                 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}2304x256 \\ charge-based \\ IMC cross-bar\end{tabular}}       & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}10 RISC-V cores,\\  DNN acc. (digital)\end{tabular}}      & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}1024x512\\  PCM-based \\ cross-bar\end{tabular}}                & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}34 256x256 analog \\ cross-bar, \\ 8 RISC-V cores, \\ depth-wise acc. (digital)\end{tabular}}    \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}IMC \\ storage \\ capability\end{tabular}}}                           & \multicolumn{2}{c|}{590 Kb}                                                                                  & \multicolumn{2}{c|}{--}                                                                                  & \multicolumn{2}{c|}{524 K cells}                                                                               & \multicolumn{2}{c}{2.2 M cells}                                                                                                             \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Peak Int.\\ Perf. {[}TOPS{]}\end{tabular}}}}          & \multicolumn{2}{c|}{2.19 (1b-1b)}                                                                            & \multicolumn{2}{c|}{0.016 (8b-8b)}                                                                       & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}2, 7.7, 26.1 \\ (8/6/4b-4b)\end{tabular}}                       & \multicolumn{2}{c}{\textbf{0.958} (8b-4b)}                                                                                                           \\
\multicolumn{1}{l|}{}                                                                                                        &                                                      & \multicolumn{1}{c|}{}                                 & \multicolumn{2}{c|}{0.032 (ML perf 8b)}                                                                  &                                                       & \multicolumn{1}{c|}{}                                  &                                                                      & \multicolumn{1}{c}{}                                                 \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Peak Int.\\ Efficiency\\ {[}TOPS/W{]}\end{tabular}}}} & \multicolumn{2}{c|}{400 (1b-1b)}                                                                             & \multicolumn{2}{c|}{0.61 (8b-8b)}                                                                        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}13.5, 45.5, 112 \\ (8/6/4b-4b)\end{tabular}}                    & \multicolumn{2}{c}{\textbf{6.39} (8b-4b)}                                                                                                            \\
\multicolumn{1}{l|}{}                                                                                                        &                                                      & \multicolumn{1}{c|}{}                                 & \multicolumn{2}{c|}{1.3 (ML perf 8b)}                                                                    &                                                       & \multicolumn{1}{c|}{}                                  &                                                                      & \multicolumn{1}{c}{}                                                 \\ \hline
\multicolumn{1}{l|}{}                                                                                                        & \multicolumn{1}{l}{}                                 & \multicolumn{1}{l|}{}                                 & \multicolumn{1}{l}{}                               & \multicolumn{1}{l|}{}                               & \multicolumn{1}{l}{}                                  & \multicolumn{1}{l|}{}                                  & \multicolumn{1}{l}{}                                                 &                                                                      \\
\multicolumn{9}{c}{\textbf{Machine Learning Workload}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Activations\\ Precision\\ (INT)\end{tabular}}}                        & \multicolumn{2}{c|}{1-8b}                                                                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}32/16/8b with cores,\\ 8b with digital acc.\end{tabular}} & \multicolumn{2}{c|}{8/6/4b}                                                                                    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}32/16/8/4/2b with cores, \\ 8b with IMA, \\ 8b with dig. Acc,\end{tabular}}                   \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Weights \\ Precision\\ (INT)\end{tabular}}}                           & \multicolumn{2}{c|}{1-8b}                                                                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}32/16/8b with cores,\\ 8b with digital acc.\end{tabular}} & \multicolumn{2}{c|}{4b}                                                                                        & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}32/16/8/4/2b with cores, \\ 4b with IMA, \\ 8b with dig. Acc,\end{tabular}}                   \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}depth-wise\\  support\end{tabular}}}                                  & \multicolumn{2}{c|}{RISC-V Core}                                                                             & \multicolumn{2}{c|}{RISC-V Cores}                                                                        & \multicolumn{2}{c|}{None}                                                                                      & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}RISC-V Cores and\\ Dedicated digital accelerator\end{tabular}}                                \\ \hline
\multicolumn{1}{l|}{\textbf{NN Model}}                                                                                       & \multicolumn{2}{c|}{9-layers CNN}                                                                            & \multicolumn{2}{c|}{MobileNetV2}                                                                         & \multicolumn{2}{c|}{AnalogNets (AN)}                                                                           & \multicolumn{2}{c}{MobileNetV2}                                                                                                             \\ \hline
\multicolumn{1}{l|}{\textbf{Tot.  Param.}}                                                                                   & \multicolumn{2}{c|}{$\sim$3.5M}                                                                              & \multicolumn{2}{c|}{2.2 M}                                                                               & \multicolumn{2}{c|}{301K (AN-KWS)}                                                                             & \multicolumn{2}{c}{2.2 M}                                                                                                                   \\
\multicolumn{1}{l|}{\textbf{}}                                                                                               &                                                      & \multicolumn{1}{c|}{}                                 &                                                    & \multicolumn{1}{c|}{}                               & \multicolumn{2}{c|}{354K (AN-VWW)}                                                                             &                                                                      & \multicolumn{1}{c}{}                                                 \\ \hline
\multicolumn{1}{l|}{\textbf{Tot. MMAC}}                                                                                      & \multicolumn{2}{c|}{Not Specified}                                                                           & \multicolumn{2}{c|}{281.6}                                                                               & \multicolumn{2}{c|}{Not Specified}                                                                             & \multicolumn{2}{c}{281.6}                                                                                                                   \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Inference \\ Perf.\end{tabular}}}}                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}176 images/s\\  (a1b-w1b)\end{tabular}}                       & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}10 frames/second\\ a8b-w8b PW and DW\end{tabular}}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}KWS: 7.762 inf/s \\ (a8b-w4b)\end{tabular}}                     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{99 frames/s} \\ (a8b-w4b PW,\\ a8b-w8b DW)\end{tabular}}                                       \\
\multicolumn{1}{l|}{}                                                                                                        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}23 images/s\\  (a4b-w4b)\end{tabular}}                        & \multicolumn{2}{c|}{}                                                                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}VWW:1.063 inf/s \\ (a8b-w4b)\end{tabular}}                      &                                                                      &                                                                      \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Inference\\ En. Eff.\end{tabular}}}}                  & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}5.31 uJ/inf \\ (a1b-w1b)\end{tabular}}                        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}1.19 mJ/frame \\ a8b-w8b PW and DW\end{tabular}}          & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}KWS: 8.22 uJ/inf \\ (a8b-w4b)\end{tabular}}                     & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{0.482 mJ/frame} \\ (a8b-w4b PW,\\ a8b-w8b DW)\end{tabular}}                                     \\
\multicolumn{1}{l|}{}                                                                                                        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}105.2 uJ/inf\\  (a4b-w4b)\end{tabular}}                       & \multicolumn{2}{c|}{}                                                                                    & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}VWW: 15.6 uJ/inf \\ (a8b-w4b)\end{tabular}}                     &                                                                      &                                                                     
\end{tabular}
\label{tab:SOA_TABLE}
\end{table*}

==> text/results_legacy.tex <==
\subsubsection{Experimental Setup}
Our results are obtained by synthesizing the cluster while varying the number of TCDM master ports in the accelerator, using Synopsys Design Compiler to target the GlobalFoundries 22nm FDX technology (SSG corner @ 0.59V and 250 MHz).
% We characterized two scenarios for performance and power: software-based execution; the second one is the power consumed while the cluster was executing a CNN layer on the IMA.
% The tool used for Synthesis is Synopsys Design Compiler, using GF22FDX libraries. The operating conditions are SSG  constraints on the clock.
For power analysis, we used Synopsys PrimeTime with typical corner with 0.65V at 25°C, with switching activity back-annotation from post-synthesis simulation. The IMA model for performance and power are estimated from~\cite{hermesCor}; each PCM device has an area of 18.2 $\mu m^2$ and a single array operation takes 70ns. We assume that the PCM array is properly sized to fit all weights. All results are reported relative to the cluster frequency of 250MHz and using the convention 1 MAC = 2 OPs.

\subsubsection{Baseline IMA performance}
\label{sec:ima_std_conv}


\begin{figure}[t]
\centerline{\includegraphics[width=0.6\textwidth]{images/old_paper/maledetta-fig3-1.pdf}}
\caption{Performance on standard convolution: Software execution (SW) vs IMA acceleration (frequency = 250MHz). The N/N configuration indicates the number of load and store master ports (32-bit each), respectively.}
\label{fig:ima_opt}
\vspace{-5mm}
\end{figure}

% \subsection{IMA results on standard convolutions}
% %  change to something like IMA perf vs TCDM bw ?
% \label{sec:ima_std_conv}
% %\textbf{Maybe move to results?}
The peak theoretical performance of the PCM array is limited only by its size: for a 100x100 array, for example, 286 GOPS are achieved; for a 1000x1000 array, this would be 28.6 TOPS, etc. However, real performance is limited by \textit{i)} array utilization; \textit{ii)} how fast activation data is streamed in/out of the IMA. To assess the IMA's performance in a realistic baseline case, we used a standard convolutional layer with 3x3 filter, with 16x16 output size, 32 input channels, and 64 output channels ($\sim$4.7 MMAC).
% 
% which can be seen in Fig.~\ref{fig:ima_opt}.
% IMA presents multiple instances where \textsc{{x/y}} indicates the number of TCDM ports configurations for input and output respectively.
% The ports have been kept symmetrical since the amount of bandwidth in input or output depends on the layer executed (in this example emphasis was mostly on stream-in).
Fig.~\ref{fig:ima_opt} shows the IMA performance obtained while sweeping the number of load/store ports from 1/1 to 16/16, compared with a pure software execution on the 8 cores using PULP-NN~\cite{garofalo2020pulp} which achieves more than 55\% utilization of the SIMD MAC units in the cores.
% 
%We notice that on standard convolutions, the main limit to the IMA performance is given by the speed at which the data can be streamed in. 
In this case, a significant portion of the execution time is due to data stream-in which can be reduced by increasing the bandwidth to the IMA.
The speed-up ranges from 10.2$\times$ on \textsc{1/1} configuration up to 36.7$\times$ when \textsc{16/16} is used.
% On the core side, most of the time is spent on executing the inner loop of the kernel while 20\% of the cycles is consumed on data marshaling (IM2COL phase, which is not required on IMA thanks to the 3D transfers of the streamers). The remaining contribution on fig~\ref{fig:ima_opt} have the following meaning: \textit{stream-in overhead} includes contentions, fifos delays, data alignment; \textit{SETUP}, which is the number of cycles required to update addresses, enabling/disabling the PCM devices between jobs.




\subsubsection{Case Study: MobilenetV2}
\label{sec:ima_depthwise}


To highlight the advantages and trade-offs of IMC on a realistic use case for extreme edge computing, we selected MobileNetV2, a widely used DNN benchmark constructed as a deep stack of units called \textit{BottleNecks}.
%\textit{
%\textbf{This text can be cut if space is scarce.}
%All BottleNecks share the same structure but differ from each other in terms of %number of in/out channels and spatial stride; their operation is based on a 1x1 %convolution used to expand tensors channel-wise by a factor of 6; a 3x3 depthwise %layer performing separate transformations on each channel; and another 1x1 %convolution compressing back the number of channels.
%Finally, the input of the BottleNeck is added to the output by means of a bypass %connection.
%}
For this analysis, we focus on the BottleNeck configuration that is shown in Fig.~\ref{fig:bottleneck}; the configuration is chosen so to fit the on-cluster TCDM (512 kB) without requiring any activation data tiling~\cite{burrello2020dory}, which is beyond the scope of this work.\footnote{We note that data tiling will further decrease energy efficiency.}
% The Bottleneck is made of several sub-layers where the first is a \textit{conv 1x1} that expands the number of channels by 6, followed by a depthwise layer and a pointwise that compress back the number of channels. The first and second layer have a \textit{RELU6} as activation function while the pointwise is only followed by a residual block that sums the output of the pointwise with the input of the bottleneck.
% In this work we consider a TCDM large enough (512 KB) to accommodate input and output features maps. Bottlenecks deeper in the network are significantly larger than the one tested and would not fit all in the TCDM requiring tiling. Studying bottlenecks that fit all in TCDM shows the maximum performance achievable with the system and the minimization of the tiling overhead is out of the scope of this work.



All layers in the BottleNeck can be mapped on the IMA. For the 1x1 convolutional layers, the mapping is direct as explained in Section~\ref{sec:execution_model}, exploiting their high-level of channel parallelism. However, in the 3x3 depthwise layer each output channel depends only on a single input channel. This fact means that optimizing at the same time the array utilization and the execution performance is not possible.

%The three layers of the bottleneck can be mapped to the IMA PCM devices directly but can be efficiently done only in convolution where the output also depends on the value across the input channels, which does not happen in the depthwise layer of the bottleneck: each channel output depends only on the values of the input at the same channel depth. This means that the input from other channels cannot be used to compute the output of the current channel requiring padding (as shown on the lower right side of  fig\ref{fig:bottleneck}). 


\begin{figure}[t!]
\centerline{\includegraphics[width=0.45\textwidth]{images/old_paper/memory_mapping_ima_2.png}}
\caption{Components of MobilenetV2 bottleneck block with stride = 1 and mapping structure in the PCM crossbar for depthwise layers. All the gray rectangles are padding required for computing more than 1 channel per job.}
\label{fig:bottleneck}
\vspace{-5mm}
\end{figure}


A $K\times K$ depthwise layer with $C$ in/out channels can be mapped as a standard layer with all weights out of a diagonal set to 0, as shown in Fig.~\ref{fig:bottleneck}. This means that out of $K^2 \times C^2$ crossbar locations, only $K^2\times C$ are useful, leading to low utilization of the array. On the other hand, the depthwise can be split in separate jobs for better array utilization, but this leads to a smaller amount of operations per job, reducing performance. The total number of crossbar elements required is in general given by $N_{xbar} = K^2 \times C_{job}^2$, where $C_{job}$ is the number of channels per job. For a MobileNet-V2, full throughput for all Bottlenecks would require a 23$\times$ larger array than what simply counting the number of parameters would suggest. This result stands even if the number of depthwise parameters is just $\sim$4\% of the total number of weights.
% Clearly, this approach is not feasible and fixing the number of output channels computed per job will allow packing weights into devices more densely, and thus provide a trade-off between PCM devices and throughput.
In this work, we considered $C_{job}=8$ and $16$ as reasonable trade-off configurations, which translates to an increase of 25\% and 54\% in the number of devices respectively. These are indicated as \textsc{ima8} and \textsc{ima16}, respectively, in the following sections.
%The throughput of depthwise layers is also hampered by the output structure from the previous layer, which is stored as HWC, meaning the feature map is stored channel first, then width and last height. Depthwise layers executed on IMA require CHW (width first) structure which translates into higher overhead for fetching the input feature map due to data not being contiguous in memory. In this case, 9 requests to memory are necessary given the 3 by 3 kernel filter even though there is enough bandwidth to fetch everything in one request. %Depending on the number of fixed output chosen, 16 or 8 different channels are fetched from memory on each memory transaction and are then offset internally.
% 


\begin{figure*}[t]
\centerline{\includegraphics[width=\textwidth]{images/old_paper/perf_results_compressed_3.png}}
\caption{Performance of several design implementations of the MobileNetV2 bottleneck. a) Performance results measured in GOPS; b) Energy efficiency in TOPS/W; c) Area efficiency in GOPS/$mm^2$. Red circles on a) and b) indicate best results.}
\label{fig:res_compressed}
\vspace{-5mm}
\end{figure*}

An alternative solution supported by the heterogeneous cluster we propose is the parallel execution of the depthwise layer via software~\cite{garofalo2020pulp} on the 8 RISC-V cores of the cluster, intermixed with IMA-based execution of 1x1 layers. This configuration, which is reported as \textsc{hybrid}, requires the parameters from the depthwise layer to be stored in memory instead of IMA which we consider a reasonable trade-off since those parameters account only for ~4\% of the total weights.
% \subsubsection{MobileNetV2 Bottlenecks Results}


The performance results in this section are from the Bottleneck with sizes reported in Fig.~\ref{fig:bottleneck} sweeping across 1 to 16 ports for stream-in and out. In Figs.~\ref{fig:res_compressed} (a-c) we can see how the benefits of adding TCDM master ports start to fall off after 4/4: the depthwise layer dominates the number of cycles (see Fig.~\ref{fig:totCycles}) and increasing ports doesn't render as sizeable an effect as shown in Fig.~\ref{fig:ima_opt}.
In particular, for the \textsc{hybrid} solution, increasing bandwidth toward IMA with more ports does not influence the depthwise execution.
In \textsc{ima16} configuration the bandwidth for depthwise saturates when all the channels can be fetched in one cycle: 4 TCDM ports of 4 bytes each are enough; going over only benefits 1x1 convolutions.
The same reasoning can be applied to 8 channels per job, where 2 ports are sufficient.

Thus, the importance of the depthwise layer in the Bottleneck drives the total improvement when using the IMA down to $\sim$3$\times$ the software implementation (down from $\sim$36$\times$ on standard convolutions).
Overall, the \textsc{hybrid} configuration stands out as the fastest: this is because even in the \textsc{ima16} configuration, the depthwise layer is slower than in software, as can be seen in Fig.~\ref{fig:totCycles}.
Similar considerations can be made with respect to energy efficiency, noticing that adding more ports than necessary reduces energy efficiency with respect to the peak at 4 (\textsc{hybrid}/\textsc{ima16}) or 2 ports (\textsc{ima8}), as it puts more pressure on the memory system.
\textcolor{blue}{From the previous }

To put in perspective the cost of increasing the throughput using IMA, the area efficiency reported in Fig~\ref{fig:res_compressed}(c) is relative to the effective area of the PCM arrays utilized to implement the Bottleneck (including padding). The \textsc{hybrid} solution has the best result requiring $\sim$3.25$\times$ and 2.13$\times$ smaller PCM area for the same bottleneck when compared to \textsc{ima16} and \textsc{ima8}, respectively. Considering also the area of the cluster itself, we obtain 1.82$\times$ and 2.56$\times$ better GOPS/$mm^2$, respectively.

% The fig~\ref{fig:res_compressed}(b) shows energy efficiency in TOPS/W. Here we see how the peak of efficiency is with 4 TCDM ports for the hybrid and IMA-16, while is 2 when looking at IMA-8. Scaling the number of TCDM master ports increases both the interconnect and IMA subsystem size in both area and power consumptions. Also, the higher bandwidth puts more pressure on the memory system rising his power consumption. The latter has a bigger impact in terms of power consumption than performance benefits hence reducing the energy efficiency.


\label{sec:bottlenecs_res}
\begin{figure}[t!]
\centerline{\includegraphics[width=0.45\textwidth]{images/Exec_cycles_different_PULP_configs_v1.pdf}}
\caption{Performance of the execution of the various Bottleneck layers: pointwise (PW)-depthwise (DW)-pointwise (PW) and the residual connection, considering different execution configurations: full software (CORES), full IMA with the two different custom configurations for DW, hybrid (DW in SW) and DW ACC, where DW is offloaded to the dedicated accelerator. Residual always computed by the cores. Explicit data marshalling (hwc to chw) only needed for SW execution of DW. The cluster runs at 250 MHz. }
\label{fig:totCycles}
\vspace{-5mm}
\end{figure}

If we compare the described \textsc{hybrid} implementation for MobileNetV2 bottleneck with a s.o.a. heterogeneous system where the IMA is integrated through a loosely-coupled 32-bit AXI bus controlled by a tiny processor \cite{jia2020programmable}, our proposed solution performs $\sim$45$\times$ better. First, our core is $\sim$10$\times$ faster on depthwise convolutions on a per-core basis. If we expand the picture to the entire cluster we would look at another $\sim$7$\times$ improvement factor. Finally, the loosely coupled integration of the IMA through a 32-bit system-bus \cite{jia2020programmable} forms a huge performance bottleneck even for standard convolutions (see Fig.~\ref{fig:ima_opt}). Our high-bandwidth tightly-coupled interconnect scheme allows delivering to the IMA the required bandwidth in a scalable way with low communication latency with the cores, improving by $\sim$3.5$\times$ the IMA performance over \cite{jia2020programmable}, making the proposed hybrid solution viable, and paving the way for a new generation of architectures exploiting synergies between analog and digital computing. Finally, the results of our exploration in Fig.\ref{fig:totCycles} suggests that further gains in the order of 10$\times$ can be achieved by extending these clusters with specialized digital accelerators better tuned for key functions of modern DNNs.

%This originates from the fact that, increasing the number of ports has a bigger impact on power consumption than on performance.
% In the fig~\ref{fig:res_compressed}(c) we report the GOPS/$mm^2$, a metric for area efficiency.

% Last graph in fig~\ref{fig:totCycles} we show the number of cycles it takes to complete the bottleneck with 4 TCDM port configurations at 250 MHz. The components are split into sections as shown in \ref{fig:bottleneck}. Dominating the computation time when using the IMA is depthwise, increasing the number of output channels reduces the number of jobs required, and it scales quite linearly given the fact that the output of the PCM crossbar requires a fixed time to evaluate the output. When looking at the convolutions 1x1, the amount of speed-up achieved is comparable with the fig~\ref{fig:ima_opt} when using the software version as reference.

